Light-Field for RF

Most computer vision systems and computational photography systems are visible light based which is a small fraction of the electromagnetic (EM) spectrum. In recent years radio frequency (RF) hardware has become more widely available, for example, many cars are equipped with a RADAR, and almost every home has a WiFi device. In the context of imaging, RF spectrum holds many advantages compared to visible light systems. In particular, in this regime, EM energy effectively interacts in different ways with matter. This property allows for many novel applications such as privacy preserving computer vision and imaging through absorbing and scattering materials in visible light such as walls. Here, we expand many of the concepts in computational photography in visible light to RF cameras. The main limitation of imaging with RF is the large wavelength that limits the imaging resolution when compared to visible light. However, the output of RF cameras is usually processed by computer vision and perception algorithms which would benefit from multi-modal sensing of the environment, and from sensing in situations in which visible light systems fail. To bridge the gap between computational photography and RF imaging, we expand the concept of light-field to RF. This work paves the way to novel computational sensing systems with RF.

==> application.tex <==
\section{Potential computational sensors}
We believe that this paper paves way for transfer and combined development of computational sensing techniques and for building important and novel computational sensing applications. We now describe two concepts that can potentially benefit from the transfer of of the computational sensing techiques across these two domains.

\subsection{Application to visible light imaging}
ToF cameras have the illumination source and the receiver are co-located and share the same clock so that the ToF measured by the camera corresponds to the actual ToF and is not affected by any clock offset between the source and the receiver. However, in a more general setting, the illumination source and the receiver need not be co-located. For example, consider ubiquitous RF system like WiFi, where a WiFi signal source like one's cellphone is different from the WiFi signal receiver like a WiFi router. 

Developing systems with decoupled source and receivers offers greater flexibility, enables novel applications and expands the kind of devices on which imaging can be enabled. It further enables multiple ToF cameras to operate simultaneously. Consider the scenario where multiple autonomous vehicles are simultaneously operating on a road. Each vehicle has its own LIDAR and RADARs and the signals interfere with each other creating extremely noisy ToF measurements with catastrophic consequences. Having a single light source on the road and if only receivers in the cars operate, then multiple autonomous vehicles can simultaneously generate maps and navigate. 

However, with it comes the challenge of recovering ToF from systems where the light source and the receiver have large clock offset that constantly drifts making the estimated ToF values error-prone and meaningless. Fortunately, due to natural constraints posed by RF cameras where the illumination source is decoupled from the receiver, the RF camera research provides a solution~\cite{kotaru2017position} that we can import to ToF cameras. The approach exploits a moving receiver and uses the fact that the clock offset affects the ToF measurements of different reflectors in the same manner to compensate for clock offset and still recover ToF.

\noindent{\textbf{ToF imaging with decoupled light source and receiver }}
Fig.~\ref{fig:tofConcept} shows a moving camera and a stationary reflectors and illumination source. $\vec{p_0}$ is the position of the light source. $\vec{\delta_t}$ is the position of the camera at time $t$. $\vec{p_n}$ is the position of the virtual source from which the signal seems to come from as the signal gets reflected from $n^\mathrm{th}$ reflector. $(\vec{r_0})_t$ and $(\vec{r_n})_t$ are the direction of the incident signal coming from the signal source and the $n^\mathrm{th}$ reflector respectively. 

As the signal has $(N-1)$ reflectors and if the camera is moved through $T+1$ positions, there are $(3T + 3N)$ unknowns, i.e., $(N)$ three-dimentional positions of real signal source/virtual sources of each of the reflectors and $T$ positions of the camera at all the time instants with respect to the position at the first time instant. The position of the camera at the first time instant determines the coordinate system. The distnace measurement of signal at time $t$ corresponding to the $n^\mathrm{th}$ reflector is 
\begin{equation}
(\vec{p_n} - \vec{\delta_t})\cdot(\vec{r_n})_t + \psi_t,
\end{equation}
assuming that the change in the position of the camera is small compared to the distance between the reflector and the camera. The direction of the incoming signal is available from the camera because the camera already captures the intensity as a function of the propagation angle. As the camer moves, the physical pixel of the reflectors gets assigned to different image pixels and has different propagation angle at the camera. $psi_t$  is the additional distance that is measured due to clock offset that is the same for the measurement obtained at all the pixels. 

Consider one of the virtual sources/source as a reference pixel. Then subtraction of ToF measurements from a reflector pixel and the measurement of the reflector pixel results in the measured relative distance of 
\begin{equation}
(\vec{p_n} - \vec{\delta_t})\cdot(\vec{r_n})_t - (\vec{p_0} - \vec{\delta_t})\cdot(\vec{r_0})_t,
\end{equation}
and voila, the clock offset term disappears. For $N$ reflectors and $T$ camera positions, we can obtain $(N-1)\times(T)$ such equations and the linear system can be solved as long as the number of equations are larger than the number of variables and the propagation angles of the signal from the reflectors are far enough from each other to generate linearly independent equations.

\begin{figure*}\label{fig:tofConcept}
\includegraphics[width=1\textwidth]{tofConcept.jpg}
  \caption{Illustration of ToF measurement in spite of of decoupled illumination source and camera}
\end{figure*}


\subsection{Application to RF light imaging}
As discussed in Sec.~\ref{sec:sensor}, the RF sensors are plagued by small number of sensors and no lens. A densely packed physical array of sensors enables capture the same physical scene with more number of pixels. This makes a large sensor array an important part of visible light cameras for high resolution. In a visible light camera, lens perform an important function of decoupling the light that is incident on the lens from all the directions so that the light from one direction falls on one photodetector alone. So, RF systems lack the most important components in visible light systems that enable high resolution imaging in visible light systems. 

By providing intensity of light coming from one direction, each pixel sensor in a traditional camera is essentially providing one specific linear combination of intensities of the pixels of the physical world. However, one does not need to have multiple pixels to provide multiple linear combinations. One can exploit sensors along other dimensions to provide multiple linear combinations, thus achieving high resolution imaging. 

For example, single pixel imagers illuminate the scene with different patterns of light and the pixel measurement obtained for each pattern provides one linear combination of intensities of light~\cite{satat2017lensless}. So, when constrained by limited physical sensor array, multiple measurements are obtained along time dimension by exploiting the use of different patterns of light illumination. 

In the absence of physical lens that maps the pixels of the physical world at different directions to different pixels of an image, computational algorithms provide a way to decouple the signal coming from different directions. In visible light domain, lensless single pixel imagers resort to compressive sensing techniques to recover the signal incident along different directions by using a linearly independent set of combinations of the intensity of the reflections from different pixels of the physical world. 

Modeling based approaches like compressive sensing are brittle and falter in the presence of mismatch between the model used for inversion and the actual model through which the measurements are formed [??]. However, the real environments are very complex with scattering, diffraction and irregular surfaces. However, models accounting for these phenomenon are very complex and attempts to solve them can be computationally intractable. So, using approximate models is results in a significant model mismatch. More recent computational imaging approaches use deep learning to overcome the `model mismatch' problem. 

\noindent{\textbf{High resolution RF imaging: }}
Imaging passive reflectors is the traditional application of imaging. Providing the intensity of the reflected RF light and the corresponding ToF of the reflectors is very useful in several applications as the absorption properties of the RF light differ significantly from visible light enabling imaging of reflectors that are occluded. For example, consider an autonomous vehicle moving through fog or imaging for concealed weapons in airports, imaging a human body for diagnostic purposes, a drone imaging the skies for traffic control with other drones. 

Radars have long been explored for RF imaging but they have mostly created images with extremely poor resolution on order of several tens of centimeters [??]. Exploiting the imaging target's motion to create multiple combinations of intensity of the the reflected light of different patches of the target reflector provides a large number of measurements provides opportunity for high resolution imaging. This process, called as Inverse Synthetic Aperture Radar (InSAR) imaging, has long been in use in imaging objects on a conveyer belt where one knows the exact trajectory of different patches of the target reflector [??]. In a more natural setting, using a ToF camera like Kinect to obtain the trajectories of different patches of the target reflector that is moving frees the system from having to rigidly attach the target to a conveyer belt whose motion is perfectly known. 

There are multiple scenarios that require imaging through an occlusion but having a camera is a strict no-no; for example monitoring gait or detecting elderly fall throughout home including bedrooms and bathrooms. Visual odometry based techniques, used in systems like Hololens, that navigate a camera by continuously taking pictures also poses a significant privacy threat. In those scenarios, instead of equipping the environment with a ToF camera like Kinect to obtain the ToF of moving reflector creating multiple measurements across time, multiple RF reflectors can be embedded into walls in the rooms that provide multiple combinations of the intensity and ToF of any target reflector. Multiple smart reflectors in the environment essentially create different patterns of reflected light creating different combinations of pixels of the physical world.


RF systems imaging a passive reflector have long been crippled by  limiting assumptions like reflectors are isotropic, i.e., the reflectivity of a reflector is the same irrespective of the viewing angle and that the reflectivity of different patched on a target reflector is the same. Different antennas, whether physical or virtual antennas caused due to motion of target or the imaging sensor itself whose motion is known, have different viewing angles of a patch on the  target reflector. Applying deep learning to transfer the series of viewing angles of different antennas and the respective measurements obtained at the antennas to recover the intensity of reflected light in RF spectrum in different patches of the target reflector provides a promising alternative that overcomes the limitations of existing algorithms that rely on simplistic assumptions.




==> arxiv_rfImaging /application.tex <==
\section{Potential computational sensors}
We believe that this paper paves way for transfer and combined development of computational sensing techniques and for building important and novel computational sensing applications. We now describe two concepts that can potentially benefit from the transfer of of the computational sensing techiques across these two domains.

\subsection{Application to visible light imaging}
ToF cameras have the illumination source and the receiver are co-located and share the same clock so that the ToF measured by the camera corresponds to the actual ToF and is not affected by any clock offset between the source and the receiver. However, in a more general setting, the illumination source and the receiver need not be co-located. For example, consider ubiquitous RF system like WiFi, where a WiFi signal source like one's cellphone is different from the WiFi signal receiver like a WiFi router. 

Developing systems with decoupled source and receivers offers greater flexibility, enables novel applications and expands the kind of devices on which imaging can be enabled. It further enables multiple ToF cameras to operate simultaneously. Consider the scenario where multiple autonomous vehicles are simultaneously operating on a road. Each vehicle has its own LIDAR and RADARs and the signals interfere with each other creating extremely noisy ToF measurements with catastrophic consequences. Having a single light source on the road and if only receivers in the cars operate, then multiple autonomous vehicles can simultaneously generate maps and navigate. 

However, with it comes the challenge of recovering ToF from systems where the light source and the receiver have large clock offset that constantly drifts making the estimated ToF values error-prone and meaningless. Fortunately, due to natural constraints posed by RF cameras where the illumination source is decoupled from the receiver, the RF camera research provides a solution~\cite{kotaru2017position} that we can import to ToF cameras. The approach exploits a moving receiver and uses the fact that the clock offset affects the ToF measurements of different reflectors in the same manner to compensate for clock offset and still recover ToF.

\noindent{\textbf{ToF imaging with decoupled light source and receiver }}
Fig.~\ref{fig:tofConcept} shows a moving camera and a stationary reflectors and illumination source. $\vec{p_0}$ is the position of the light source. $\vec{\delta_t}$ is the position of the camera at time $t$. $\vec{p_n}$ is the position of the virtual source from which the signal seems to come from as the signal gets reflected from $n^\mathrm{th}$ reflector. $(\vec{r_0})_t$ and $(\vec{r_n})_t$ are the direction of the incident signal coming from the signal source and the $n^\mathrm{th}$ reflector respectively. 

As the signal has $(N-1)$ reflectors and if the camera is moved through $T+1$ positions, there are $(3T + 3N)$ unknowns, i.e., $(N)$ three-dimentional positions of real signal source/virtual sources of each of the reflectors and $T$ positions of the camera at all the time instants with respect to the position at the first time instant. The position of the camera at the first time instant determines the coordinate system. The distnace measurement of signal at time $t$ corresponding to the $n^\mathrm{th}$ reflector is 
\begin{equation}
(\vec{p_n} - \vec{\delta_t})\cdot(\vec{r_n})_t + \psi_t,
\end{equation}
assuming that the change in the position of the camera is small compared to the distance between the reflector and the camera. The direction of the incoming signal is available from the camera because the camera already captures the intensity as a function of the propagation angle. As the camer moves, the physical pixel of the reflectors gets assigned to different image pixels and has different propagation angle at the camera. $psi_t$  is the additional distance that is measured due to clock offset that is the same for the measurement obtained at all the pixels. 

Consider one of the virtual sources/source as a reference pixel. Then subtraction of ToF measurements from a reflector pixel and the measurement of the reflector pixel results in the measured relative distance of 
\begin{equation}
(\vec{p_n} - \vec{\delta_t})\cdot(\vec{r_n})_t - (\vec{p_0} - \vec{\delta_t})\cdot(\vec{r_0})_t,
\end{equation}
and voila, the clock offset term disappears. For $N$ reflectors and $T$ camera positions, we can obtain $(N-1)\times(T)$ such equations and the linear system can be solved as long as the number of equations are larger than the number of variables and the propagation angles of the signal from the reflectors are far enough from each other to generate linearly independent equations.

\begin{figure*}\label{fig:tofConcept}
\includegraphics[width=1\textwidth]{tofConcept.jpg}
  \caption{Illustration of ToF measurement in spite of of decoupled illumination source and camera}
\end{figure*}


\subsection{Application to RF light imaging}
As discussed in Sec.~\ref{sec:sensor}, the RF sensors are plagued by small number of sensors and no lens. A densely packed physical array of sensors enables capture the same physical scene with more number of pixels. This makes a large sensor array an important part of visible light cameras for high resolution. In a visible light camera, lens perform an important function of decoupling the light that is incident on the lens from all the directions so that the light from one direction falls on one photodetector alone. So, RF systems lack the most important components in visible light systems that enable high resolution imaging in visible light systems. 

By providing intensity of light coming from one direction, each pixel sensor in a traditional camera is essentially providing one specific linear combination of intensities of the pixels of the physical world. However, one does not need to have multiple pixels to provide multiple linear combinations. One can exploit sensors along other dimensions to provide multiple linear combinations, thus achieving high resolution imaging. 

For example, single pixel imagers illuminate the scene with different patterns of light and the pixel measurement obtained for each pattern provides one linear combination of intensities of light~\cite{satat2017lensless}. So, when constrained by limited physical sensor array, multiple measurements are obtained along time dimension by exploiting the use of different patterns of light illumination. 

In the absence of physical lens that maps the pixels of the physical world at different directions to different pixels of an image, computational algorithms provide a way to decouple the signal coming from different directions. In visible light domain, lensless single pixel imagers resort to compressive sensing techniques to recover the signal incident along different directions by using a linearly independent set of combinations of the intensity of the reflections from different pixels of the physical world. 

Modeling based approaches like compressive sensing are brittle and falter in the presence of mismatch between the model used for inversion and the actual model through which the measurements are formed [??]. However, the real environments are very complex with scattering, diffraction and irregular surfaces. However, models accounting for these phenomenon are very complex and attempts to solve them can be computationally intractable. So, using approximate models is results in a significant model mismatch. More recent computational imaging approaches use deep learning to overcome the `model mismatch' problem. 

\noindent{\textbf{High resolution RF imaging: }}
Imaging passive reflectors is the traditional application of imaging. Providing the intensity of the reflected RF light and the corresponding ToF of the reflectors is very useful in several applications as the absorption properties of the RF light differ significantly from visible light enabling imaging of reflectors that are occluded. For example, consider an autonomous vehicle moving through fog or imaging for concealed weapons in airports, imaging a human body for diagnostic purposes, a drone imaging the skies for traffic control with other drones. 

Radars have long been explored for RF imaging but they have mostly created images with extremely poor resolution on order of several tens of centimeters [??]. Exploiting the imaging target's motion to create multiple combinations of intensity of the the reflected light of different patches of the target reflector provides a large number of measurements provides opportunity for high resolution imaging. This process, called as Inverse Synthetic Aperture Radar (InSAR) imaging, has long been in use in imaging objects on a conveyer belt where one knows the exact trajectory of different patches of the target reflector [??]. In a more natural setting, using a ToF camera like Kinect to obtain the trajectories of different patches of the target reflector that is moving frees the system from having to rigidly attach the target to a conveyer belt whose motion is perfectly known. 

There are multiple scenarios that require imaging through an occlusion but having a camera is a strict no-no; for example monitoring gait or detecting elderly fall throughout home including bedrooms and bathrooms. Visual odometry based techniques, used in systems like Hololens, that navigate a camera by continuously taking pictures also poses a significant privacy threat. In those scenarios, instead of equipping the environment with a ToF camera like Kinect to obtain the ToF of moving reflector creating multiple measurements across time, multiple RF reflectors can be embedded into walls in the rooms that provide multiple combinations of the intensity and ToF of any target reflector. Multiple smart reflectors in the environment essentially create different patterns of reflected light creating different combinations of pixels of the physical world.


RF systems imaging a passive reflector have long been crippled by  limiting assumptions like reflectors are isotropic, i.e., the reflectivity of a reflector is the same irrespective of the viewing angle and that the reflectivity of different patched on a target reflector is the same. Different antennas, whether physical or virtual antennas caused due to motion of target or the imaging sensor itself whose motion is known, have different viewing angles of a patch on the  target reflector. Applying deep learning to transfer the series of viewing angles of different antennas and the respective measurements obtained at the antennas to recover the intensity of reflected light in RF spectrum in different patches of the target reflector provides a promising alternative that overcomes the limitations of existing algorithms that rely on simplistic assumptions.




==> arxiv_rfImaging /camera.tex <==
\section{Plenoptic Function}\label{sec:lightField}
Light emitted from a signal source travels through the environment and interacts with it. The plenoptic function~\cite{adelson1991plenoptic} is a useful tool to describe light transport. Similarly, a RF plenoptic function is helpful when thinking about RF systems. For completeness, we provide a brief introduction to the concepts of the plenoptic function in optical frequencies. In general, we can describe the light field as the real-valued high-dimensional function:
\begin{equation}
L(x,y,z, \xi, \psi, t, f)
\end{equation}
where $x,y,z$ are the spatial coordinates, $\xi$ and $\psi$ are the azimuth and elevation angles of propagation respectively, $t$ is time, $f$ represents the optical frequency. $L(x,y,z, \xi, \psi, t, f)$ is a measure of the radiance of a ray traveling along the direction dictated by the angles of propagation, at a point in space dictated by the spatial coordinates, at time $t$, carrying a signal of frequency $f$.


The underlying concepts of the plenoptic function in optical frequencies are useful in the RF spectra as well. In this case it is useful to think about wavefronts as opposed to light rays. For example, the angular components now describe the normal to the local wavefront. Also, unlike visible light sources most of which emit incoherent light, most of the RF sources generate coherent signal. In visible light systems, unless the source is a laser producing coherent light, the emitted light contains waves with all possible phase values resulting in a transmitted signal that has no useful phase information. Similarly, typical visible light sensors can only measure the intensity and radiance of the incident light. So, using a real-valued plenoptic function, that ignores phase, to describe the radiance of light is sufficient for visible light based systems. In contrast, most of the RF systems generate coherent waves that are in phase with each other at the signal source. 

The complex-valued RF signal, containing both amplitude and phase, as a function of three-dimensional position, two-dimensional propagation angle, time and frequency is surprisingly amenable to mathematical treatment similar to that of light plenoptic function. We call this the RF plenoptic function $L(x,y,z, \xi, \psi, t, f)$. $L(x,y,z, \xi, \psi, t, f)$ is the complex RF signal at a point $(x,y,z)$, whose normal at the local wavefront at those spatial coordinates is pointing along the direction dictated by the azimuth and elevation angles $\xi$ and $\psi$ respectively, at time $t$, carrying a signal of frequency $f$. Note that unlike light plenoptic function which is real-valued, RF plenoptic function is complex-valued. Fig.~\ref{fig:spherical} shows an example plenoptic function for a simple scenario of a spherical wave propagating in space.


\begin{figure}
  \centering
      \includegraphics[width=0.9\linewidth]{./figures/wavefront}
  \caption{An example illustration of RF plenoptic function. (Left) Illustration of spherical wavefront and rays on a two-dimensional plane. (Right) The amplitude of RF plenoptic function as a function of two of the input variables -- the x coordinate and angle of propagation.}
  \label{fig:spherical}
\end{figure}


%\section{RF Imaging sensors}
%\textbf{Camera:} A traditional 2D camera captures the intensity of the light incident at the location of a camera as a function of the direction of the incoming light. And the representation $I(x,y)$ of the intensity against a two dimensional Cartesian coordinate system is the representation of image that we are most familiar with. The cameras have evolved to capture the time of flight of the light to reach the camera from the illumination source along each direction enabling the identification of depth of the reflectors along each direction. The cameras have further evolved to even capture the entire time profile of light as it travels from the illumination source to the camera instead of capturing just a just single time of flight. The resultant image $I(x,y,t)$ captures the intensity of light in different directions as a function of time. These images $I(x,y,t)$ are no longer direct representation of what is captured by the sensors but are \textit{computed} and used for machine vision. 
%
%\textbf{Pixels: }Pixels are the sensing elements of a camera. They are sensitive to light in specific wavelengths they are designed for. A simple pixel simply integrates the light incident on it from all the directions across time and produces a current that generates a single reading or measurement. In the typical digital visible-light cameras that we are most familiar with, each pixel is a simple photodetector and a typical camera consists of millions of them in a 2D array. In general notation, the term `pixels' is also used to denote the coordinates in the final image representation and also to denote the patches of the physical world the light from which is directed to be incident on a particular pixel sensor.
%
%\textbf{Lens: }A lens transforms the incident light that is coming from all directions so that light from one direction is incident on only one pixel. Low-quality lens direct the light incident along a particular direction on multiple pixels resulting in blurred low-resolution images. A lens essentially performs the job of mapping the pixels of the physical world to the pixel sensors of the camera. In the absence of a lens, the pixel sensors generate measurements that are a result of the superposition of signals along all directions at the location of each pixel resulting in an image that is not interpretable for humans.
%
%\textbf{RF Camera: }A typical RF sensor consists of a 1D, 2D, or 3D array of antennas which are the pixel sensors of RF. An antenna with an accompanying circuit performs a similar operation as a photodetector measuring the incident RF light at the antenna from all the directions across time and generating a  reading. 
%
%It is impractical to build a high-quality lens in RF spectrum due to large wavelengths of RF light. So, there is no mapping structure like in visible light cameras that maps the pixels of the physical world to the pixel sensors in the camera. Each pixel sensor measures the superposition of RF light incident on it along all the directions. 
%
%Unlike visible light sensors where millions of pixels can be manufactured in CCD/CMOS arrays, RF spectrum lacks similar processes that help manufacturing large arrays of RF pixel sensors. This is the reason why the number of antennas in RF communication devices is limited to two or three antennas, and even in research prototypes, the number of antennas is limited to few tens of antennas. It is very hard to build RF systems with thousands or millions of antennas/pixel sensors.
%
%The goal of a RF camera is to \textit{compute} high resolution images $I(x,y,t)$ which enables several novel and important applications in autonomous driving, medical sensing, robotics, physical security and extended reality.

\section{Camera}\label{sec:sensor}
\textbf{Image: }An image captured by a camera is a projection of the plenoptic function. A pinhole camera captures a 2D projection of the plenoptic function $L(x_0,y_0,z_0, \xi, \psi, t_0)$ where $(x_0,y_0,z_0)$ is the position of pinhole, $t_0$ is the time of acquisition and the plenoptic function is integrated over all the frequencies. So, the captured image is just a function of propagation angles $\xi$ and $\psi$. Similarly, traditional and ubiquitous visible light cameras are 2D sensor arrays and generate a 2D projection of the plenoptic function:
\begin{itemize}
\item Each sensor integrates over all angles defined by the camera aperture. 
\item The depth information is lost in the projection of the scene on the sensor. 

\item The camera integrates over time during the exposure. 
\item A Bayer mask is used to sample different wavelengths (usually, these filters are broad such that each pixel integrates over a fraction of the spectrum). 
\end{itemize} 

There are many variants to the traditional camera. For example, a light-field camera captures the angular information (usually at the cost of reduced spatial resolution). A spectrometer provides high spectral resolution (at the cost of spatial information). Ultrafast cameras provides high temporal resolution and so on. 

In general, due to technological limitations only a few parameters of the plenoptic function can be sampled with high resolution. The choice of the important parameters is determined by the application. For example, in traditional cameras the spatial coordinates are sampled with high resolution.

Due to significant difference between optical and radio frequencies and the resulting differences in visible light and RF camera systems, our ability to sample the RF plenoptic function is substantially different. RF camera samples the complex-valued RF plenoptic function generating complex-valued measurements. The projection captured by an RF camera, e.g. a WiFi receiver, can be written as $L(x_k,y_k,z_k, f)$:
 \begin{itemize}
\item RF camera has a sensor array consisting of $K$ sensors and $(x_k,y_k,z_k)$ is the position of $k^{\mathrm{th}}$ sensor.
\item The sensors are typically omni-directional. Each sensor integrates over all the propagation angles. So, unlike visible light cameras, angle dependent information of the plenoptic function is completely lost. 
\item The camera integrates over time. 
\item A RF filter is used to isolate the signal from each of the constituent frequencies $f$. 
\end{itemize} 


\textbf{Pixels: }Pixels are the sensing elements of a camera. A photodector is the sensing element of a visible light camera. It integrates the light incident on it from all the directions within its field of view across time and produces a current that generates a single reading or measurement. RF Pixels are antennas with accompanying circuits that perform a similar operation as a photodetector measuring the incident RF signal at the antenna from all the directions across time and generating a reading. The antennas can be arranged in 1D, 2D, or 3D structures. RF pixels have a much larger field of view than photodetectors. For example, antennas used in typical RF systems like WiFi in smartphones are omni-directional, i.e., they have a 360 degree field of view in azimuthal direction.

Unlike visible light cameras where millions of pixels can be manufactured in CCD/CMOS arrays, RF spectrum lacks similar processes to manufacture large arrays of RF pixel sensors. Further, the size of RF antennas are comparable to the wavelength and the associated circuitry for filtering and sampling is complex. As a result it is very challenging to create dense array of RF pixels. So, unlike visible light cameras which are equipped with millions of pixels, typical RF cameras are equipped with 3-4 RF pixels. On the other hand, RF pixels measure the phase of the signal in addition to amplitude and the integration times are much shorter.


\textbf{Lens: }An important aspect of imaging in optical frequencies is the use of a lens. A lens transforms the incident light that is coming from all directions such that light from one focused target position is incident on only one pixel. The lens effectively creates a mapping between spatial coordinates in the scene to pixels on the sensor array. More specifically its a projection  $\Pi(x,y,z) \rightarrow (\bar{x},\bar{y})$. If the object is planar, parallel to the aperture, and focused by the lens then the mapping is one-to-one.

It is impractical to build a high-quality lens in RF spectrum due to large wavelengths of RF waves. So, there is no structure like in visible light cameras that maps the positions of the physical world to the pixels in the camera. Thus, we cannot sample RF plenoptic function as a function of propagation angle and each pixel integrates the RF signal incident on it from all the directions. 



In summary, RF and traditional cameras compliment each other in the way they sample the plenoptic function. Traditional cameras provide high sampling rates of the spatial coordinates, with poor spectral and phase information. RF cameras on the other hand provides a sparse measurement of the spatial coordinates, but provide high sampling rate of time (frequency) and phase. Another key difference is the lack of a lens in RF; all the signals from different angular coordinates in the scene contribute to the signal measured by an RF pixel.





%\section{Image Formation Model}
%The plenoptic function~\cite{adelson1991plenoptic} is a useful tool to describe light transport. Similarly, it is helpful when thinking about RF camera. For completeness, we provide a brief introduction to the concepts of the plenoptic function in optical frequencies. In general, we can describe the light field as the high dimensional function:
%\begin{equation}
%L(x,y,z, \theta, \psi, t, f, \phi)
%\end{equation}
%where $x,y,z$ are the spatial coordinates, $\theta$ and $\psi$ are the angles of propagation, $t$ is time, $f$ represents the optical frequency, and $\phi$ is the phase of the optical frequency (cannot be directly measured in optical frequencies). 
%
%Traditional cameras are a 2D sensor array that samples and integrates over the light field:
%\begin{itemize}
%\item The $z$ coordinate is lost or projected on the $x,y$ coordinates (depends on the camera projection model). 
%\item Each pixel integrates over all angles that enter the camera aperture. \item The camera integrates over time during the exposure. 
%\item A Bayer mask is used to sample different wavelengths (usually, these filters are broad such that each pixel integrates over a fraction of the spectrum). 
%\item The optical phase is integrated. 
%\end{itemize}
%
%There are many variants to the traditional camera. For example, a light-field camera captures the angular information (usually at the cost of reduced spatial resolution). A spectrometer provides high spectral resolution (at the cost of spatial information). Ultrafast cameras provides high temporal resolution and so on. 
%
%In general, due to technological limitations only a few parameters of the plenoptic function can be sampled with high resolution. The choice of the important parameters is a determined by the application. For example, in traditional cameras the spatial coordinates are sampled with high resolution.
%
%Another important aspect of imaging in optical frequencies is the use of a lens. The lens effectively creates a mapping between spatial coordinates in the scene to pixels on the sensor array. More specifically its a projection  $\Pi(x,y,z) \rightarrow (\bar{x},\bar{y})$. If the object is planar, parallel to the aperture, and focused by the lens then the mapping is one-to-one.
%
%\subsection{RF Plenoptic Function}
%The underlying concepts of the plenoptic function in optical frequencies are useful in the RF spectra as well. In this case it is useful to think about wavefronts as opposed to light rays. For example, the angular components now describe the normal to the local wavefront. 
%
%Due to significant difference between optical and radio frequencies our ability to sample the RF plenoptic function is substantially different. It is also common to use the frequencies instead of wavelengths in this regime of the electromagnetic spectrum.
%
%RF Pixels are antennas. These can be arranged in 1D, 2D, or 3D structures. The size of these antennas are comparable to the wavelength. As a result it is very challenging to create dense array of RF pixels. Moreover, because we don't have lenses that affect RF we cannot sample angles. Thus, RF antennas integrate over all angels. On the other side, RF antennas are sensitive and fast enough to directly measure the frequency and carrier phase at relatively short integration times. 
%
%Thus, RF and traditional cameras compliment each other in the way they sample the plenoptic function. Traditional cameras provide high sampling rates of the spatial coordinates, with poor spectral and phase information. RF cameras on the other hand provides a sparse measurement of the spatial coordinates, but provide high sampling rate of time (frequency) and phase. Both systems integrate over angular information. Another key difference is the lack of a lens in RF, as a result we are required to computationally focus or raster scan the scene.
%





==> arxiv_rfImaging /compare.tex <==
\begin{table*}[ht]
\begin{center}
    \caption{Comparison of visible light and RF sensors}
\label{compare}

\small{
    \begin{tabular}{ | p{3.8cm} | p{6.0cm} |  p{6.8cm} |}
    \hline
    & \textbf{Visible light} & \textbf{RF } \\ \hline
    Wavelength & 100s of nms & few cms \\ \hline
    \textbf{Camera} &  & \\ \hline
    Plenoptic function & $L(x,y,z, \xi, \psi, t, f)$, real-valued intensity  & $L(x,y,z, \xi, \psi, t, f)$, complex-valued  amplitude  \\ \hline 
    
    Image & projection of plenoptic function & $L(x_k, y_k, z_k, f)$ \\ \hline

    Sensors & 	 Photodetectors  & Antennas \\ \hline
    
    Field of view & Small & Large; typically omni-directional in azimuth angle \\ \hline
    
    Number of sensors & Few millions & 3-4 in conventional devices \\ \hline
    
    Lens & 	 Yes & No \\ \hline
    
    \textbf{Emitter} &  & \\ \hline
    Coherence & Typically incoherent sources; Lasers are coherent & Coherent sources \\ \hline
    
        
     Generated signal & $A x(t)$; $A$ and $x(t)$ are real-valued; $A$ is intensity & $ A \mathrm{e}^{i 2 \pi f_c t } x(t)$, $A$ and $x(t)$ are complex-valued; $A$ is complex amplitude \\ \hline
        
    Carrier frequency  & few 100s of THz & few GHz \\ \hline
    
    
    
    \textbf{Light Field transformation} &  & \\ \hline
    
    Free space propagation & $\frac{A}{r^2} x(t - \frac{r}{c})$  &  $\frac{A}{r} \mathrm{e}^{ i2 \pi f t} \mathrm{e}^{- i2 \pi \frac{r}{\lambda}}$ \\ \hline
    
    BRDF of small light patches & complex function of incoming and outgoing propagation angles; real-valued  &  $\alpha S \cos(\theta) $; complex-valued \\ \hline
    
    % Iterative reflection & $L[k,t] = E[k,t] + \sum_j g[k,j]\rho[k,j] L\big[j, t-\frac{d_{kj}}{c} \big]$ ;  $g[k,j] = \frac{1}{d^2_{kj}}$ is patch $k$ is visible from patch $j$   & $L[k,t] = E[k,t] + \sum_j g[k,j]\rho[k,j] L\big[j, t-\frac{d_{kj}}{c} \big]$; $g[k,j] = \frac{1}{d_{kj}}$ is patch $k$ is visible from patch $j$ \\ \hline
  
    
    
     \textbf{Receiver} &  & \\ \hline
    
    Image &  $ \int_T  L[x_k, y_k, z_k, \xi, \psi, t, f]$   & $ \int_T \big( \int_{\theta,\psi} L[x_k, y_k, z_k, \xi, \psi, t, f]  \big) \mathrm{e}^{-i2\pi f t - \phi}$ \\ \hline
    
    Carrier phase & Only phase difference is measurable with coherent sources, e.g., in OCT  & Measured \\ \hline
    
    Exposure time & few milliseconds & microseconds \\ \hline
    
    
    \end{tabular}
}
    
\end{center}
\end{table*}


























% \begin{table*}[ht]
% \begin{center}
%     \caption{Comparison of ToF camera and RF camera}
% \label{compare}

% \small{
%     \begin{tabular}{ | p{3.8cm} | p{6.0cm} |  p{6.8cm} |}
%     \hline
%     & \textbf{ToF camera} & \textbf{RF camera} \\ \hline

%     Generated signal & $A x(t)$; $A$ and $x(t)$ are real-valued; $A$ is radiance & $ A \mathrm{e}^{i 2 \pi f_c t } x(t)$, $A$ and $x(t)$ are complex-valued; $A$ is complex amplitude \\ \hline
    
    % Modulation  & intensity only & Both amplitude and phase \\ \hline
    
%     Modulation frequencies & 10s of MHz for ToF cameras & 10s of MHz for WiFi; few GHz for radar \\ \hline
   
%     Image formation  & demodulation and low-pass filtering & Demodulation and low-pass filtering \\ \hline
    
%     Image &  $I(f) = \int_T  L[t]  \sin(2\pi ft + \phi)$  & $I(f) = \int_T \big( \int_{\xi,\psi} L[t]  \big) \mathrm{e}^{-i2\pi f t - \phi}$ \\ \hline
    
%     Relative phase $\phi$ & known and accurately controlled & 0 in radars, unknown if the emitter and receiver are on separate devices \\ \hline
    
    
%     \end{tabular}
% }
    
% \end{center}
% \end{table*}


==> arxiv_rfImaging /conclusion.tex <==
\section{Discussion}


We presented the fundamentals towards exploiting computational photography concepts in RF cameras. The current formulation does not account for several interactions. We plan to explore the following limitations in a future work:
\begin{itemize}
    \item \textbf{Scattering:} In the interaction with reflectors, we assumed a simple  model for reflectance function that does not account for any sub-surface scattering. Another example is the lack of scattering in the propagation model.
    
    \item \textbf{Polarization:} We assumed the RF light-field is a scalar and ignored polarization effects. In practice, different materials and interactions may change the polarization state of the RF light-field.
    
    \item \textbf{Non linear interactions:} Certain reflectors may change the frequency of the emitted RF light-field. Here, we assumed that the frequency parameter does not change throughout the interactions.
\end{itemize}

In summary, we proposed the RF light-field that expands the concept of the Plenoptic function to RF. We developed several transformations including emission, propagation, interaction, and detection in RF as well as a rendering procedure for RF. Several fundamental imaging dynamics were demonstrated such as imaging resolution as a function of aperture size and system bandwidth. 

==> arxiv_rfImaging /emission.tex <==
\section{Emitter}\label{sec:source}
Many RF imaging systems employ active emitters to gain advantage in terms of improving the signal strength and reducing the interference from the ambient sources. RF sources can be broadly classified into three classes:

\noindent\textbf{Continuous wave based: }These sources emit RF light-field with single frequency. This frequency is called as carrier frequency.  Examples of continuous wave sources include Doppler radars used for identifying the speed of moving cars.

\noindent\textbf{Discrete frequency based: }RF light-field emitted from these sources consists of multiple discrete frequencies. Examples include WiFi systems.

\noindent\textbf{Pulse based: }These sources emit short pulses in radio frequency range of electromagnetic spectrum. Examples include pulse-Doppler radars used for see-through-wall applications. 

Signal generated by any RF emitter can be mathematically represented as $A\mathrm{e}^{ i2 \pi f_c t } x(t)$. $f_c$ is called as the carrier frequency. The carrier frequency is in the radio frequency portion of electromagnetic spectrum, i.e., between 3~kHz and 300~GHz. $A$ is the complex amplitude of the carrier wave. $x(t)$ is the modulating signal that is modulated over the carrier wave. In continuous wave sources, $x(t)$ is just a constant function. In discrete frequency sources, $x(t)$ is sum of complex sinusoidal signals belonging to a small number of frequencies. In pulse emitters, $x(t)$ is a short, time-limited pulse. Fig.~\ref{fig:emitter} illustrates representative RF signal emitted by these different kinds of sources. Bandwidth of the modulating signal is system-dependent. For example, modulation frequencies used in WiFi are on the order of few 10s of MHz and the bandwidth of the modulating signal used in pulse-Doppler radars is few GHz.


\begin{figure}
  \centering
      \includegraphics[width=1\linewidth]{./figures/emission}
  \caption{Illustration of signals used in continuous wave RF sources (Left), discrete frequency based sources (Middle) and pulse emitters (Right). Only the real part of the signal is shown.}
  \label{fig:emitter}
\end{figure}

The complex-valued modulating signal $x(t)$ can be decomposed into its constituent Fourier frequency components. In environments which exclusively consist of objects that do not change the frequency of the incident RF light-field, each frequency can be considered separately. In the following sections, each frequency $f$ constituting the emitted signal $A\mathrm{e}^{ i2 \pi f_c t } x(t)$ is considered separately and the corresponding wavelength is denoted by $\lambda$.

\subsection{Relation to active emission in visible light systems}\label{sec:emitLight}
The mathematical representation of signals generated by RF emitters is very similar to that used for describing active illuminators in Time-of-Flight (ToF) cameras. The light generated by these emitters can be represented as $A x(t)$. Since typical light sources, including those used in ToF cameras, are incoherent, the carrier phase term, $\mathrm{e}^{ i2 \pi f_c t }$, is absent. Further, $A$ represents the intensity emitted by the source rather than the amplitude. The modulating signal $x(t)$ is composed of a single modulating frequency, $(1 + \sin(2 \pi f t ) )$~\cite{heide2015doppler}. Note that $x(t)$ modulates amplitude of carrier signal but not the phase. The modulation frequency $f$ is on the order of 10s of MHz for ToF cameras. In pulsed laser ToF systems, $x(t)$ is a pulse with a bandwidth of few hundreds of GHz.





==> arxiv_rfImaging /intro.tex <==
\section{Introduction}
\IEEEPARstart{T}{raditional} computer vision and computational photography systems are primarily visible light based. This biased focus can be attributed to the sensitivity of our eyes to electromagnetic (EM) energy in the visible spectra, the availability of high quality lenses and dense array of detectors (pixels), and the relatively short wavelength of visible light which results in high resolution images. In parallel to the development of visible light computer vision systems, radio frequency (RF) imaging systems were developed. RF systems are mainly used for communication purposes, and in the form of RADAR for localization, tracking, and velocity estimation. In recent years RF systems have become widely used  e.g. in cars and homes, which motivates the development of imaging solutions in RF. Here, we expand many of the concepts developed for visible light to RF spectrum towards RF cameras.



Imaging with RF holds many applications that challenge computer vision with visible light. Privacy is a significant challenge for many computer vision systems, but it is easily solved with RF since no identifying or exposing information are captured. Visible light is absorbed by many materials that are transparent in RF, thus imaging through occlusions such as walls is easier in RF. Finally, many computer vision systems are safety critical and require redundancy in the form of sensing hardware and perception algorithms. Such redundancy can be achieved by fusing visible light cameras and RF cameras.

Visible light and RF share many properties as they are both EM waves. However, due to the significant difference in wavelength, there are many practical differences for the purposes of imaging. These differences can be considered as a limitation or an advantage depending on the application:

\begin{itemize}
\item Interaction with matter - for example, RF is mostly sensitive to bulk properties of objects, while visible light is sensitive to finer features. This makes it harder to distinguish among different materials with RF. On the other hand, RF propagates through materials that absorb in visible light such as walls.

\item In RF we can easily measure the phase of the wavefront. This is essential since we don't have focusing elements in RF like lenses. Thus, only bare sensor imaging is possible which is fundamentally easier with phase measurement.

\item With RF we can easily measure depth and speed of objects.

\item Due to the larger wavelength of RF, pixels (detectors) are relatively large which limits our ability to construct dense and high resolution sensor arrays.

\end{itemize}

\begin{figure}
  \centering
    \includegraphics[width=1\linewidth]{./figures/systemFig}
      \caption{Light-field for RF cameras. We propose a Plenoptic function formulation for RF including  emission,propagation, interaction with planar surfaces, and a rendering technique for RF systems.}
      \label{fig:system}
\end{figure}

\input{compare}

Many imaging applications using RF have been demonstrated, however they are application specific (e.g.~\cite{charvat2015time, adib2015capturing}). Here we take a broader approach and discuss, from first principles, the mathematical similarities and concepts describing RF and visible light cameras. We summarize these concepts in Table~\ref{compare}.



This paper highlights the differences and trade-offs between RF and visible light when considering imaging with RF systems. We build upon many of the advances in the computer vision and computational photography communities and expand many of the concepts developed primarily for visible light into RF cameras. The main contributions of our work are:

\begin{itemize}
\item A RF plenoptic function light-field formulation.
%\item RF light field transformations including emission and propagation.
\item A light-field transformation for RF that explores the complete path including emission, propagation, interaction with planar surfaces, and array based sensing.

\item A rendering solution for RF systems that accounts for wave effects, without the complexity of specialized simulators. 
\end{itemize}


We first define the notions of RF plenoptic function and RF camera in Sec.~\ref{sec:lightField} and Sec.~\ref{sec:sensor} respectively. As shown in Fig.~\ref{fig:system}, any RF imaging system consists of five components: 1) emission of RF light-field, 2) propagation through free space, 3) transformation of RF light-field as it interacts with objects in the environment, 4) propagation to a receiver, and 5) reception and processing of RF light-field resulting in the RF image. These phenomena are described in Sec.~\ref{sec:source}-Sec.~\ref{sec:receiver}. We conclude with an analysis of the resolution of images that can be obtained from an RF camera in Sec.~\ref{sec:resolution}. 



%unified mathematical and conceptual framework for describing sensing systems and image formation in both visible-light and RF spectrum. By highlighting the similarities and differences between the RF-light and visible-light based systems with respect to the same conceptual framework, we believe that this paper paves way for transfer and combined development of computational sensing techniques and for building important and novel computational sensing applications. 














%Emerging applications like autonomous driving requires the robots to see through fog, see through obstacles like corners and see in the dark, see in ways that traditional visible light sensors cannot. High-resolution sensors that can sense in the non-visible spectrums of light with different absorption properties allow us to see in these new ways and have potential to revolutionize the fields of healthcare, autonomous vehicles, physical security, robotics and extended reality. 
%
%The key challenge in achieving this vision is bypassing the lens and large sensor arrays that are critical components for achieving high resolution visible-light sensing today. Large sensor arrays allow us to capture the pixels of the physical world in a dense manner enabling us to achieve high resolution. A lens performs the important function of decoupling the overall light coming from all directions so that the pixels in the physical world map to pixels in the image.
%
%We hypothesize to \textit{expand high-resolution sensing across the electro-magnetic spectrum by building computational sensing systems over lensless, miniature-sensor arrays}. Our hypothesis is based on two key insights. In the presence of a small physical array, we can exploit sensing along other dimensions like multiple frequencies of illumination. To conquer the absence of lens, we can deploy deep learning based computational algorithms that directly map the sensor measurements to pixels of the physical world.
%
%We substantiate the hypothesis through emerging research works in a representative non-visible spectrum of light with significantly different absorption properties than light, Radio Frequency (RF) spectrum. In the process, we explore the similarities and differences in propagation, sensors and computational imaging techniques used in visible light systems and radio frequency systems.


%Signal generation, sensing mechanism and image formation in visible light systems like typical cameras and RF light systems like WiFi have interesting parallels. We describe the signal generation in visible light and RF-light systems in Sec.~\ref{sec:source} and introduce the concept of RF plenoptic function in Sec.~\ref{sec:lightField}. Sec.~\ref{sec:sensor} describes the cameras and RF cameras. We end with two examples of how we can transfer the computational sensing techniques across the two spectrums.



























%\section{Image formation model}\label{sec:model}
%
%
%\subsection{Free space propagation}
%The light emitted from a point source, whether it is RF light or visible light, follow the same inverse square law as the signal propagates through phase. The amplitude of the signal falls off as $1/r$, where the $r$ is the distance traveled by the light in the free space, whether it is RF light or visible light. The phase of the signal changes by $2 \pi f' r /c$ where $c$ is the speed of light and $f'$ is the frequency of the signal that can be modulated. 
%
%Since in visible light, only the amplitude can be modulated, the frequency value $f'$ that should be considered is the amplitude modulation frequency $f$. In RF light, both the amplitude and the phase of of carrier signal can be modulated, the frequency value $f'$ that should be considered is $f_c + f$. So, the light at a distance $r$ from light source which is modulating the amplitude with a frequency $f$ is written as $\frac{1}{r} a_f \sin(2 \pi f t + \phi - 2 \pi f \frac{r}{c})$. The RF light at a distance $r$ from the RF light source is $\frac{1}{r} a_f \mathrm{e}^{(2 \pi (f_c + f) t + \phi - 2 \pi (f_c + f) \frac{r}{c})}$. We can write a similar equation for all the modulation frequencies that constitute the emitted RF light.
%
%\subsection{RF light field}
%Ray propagation model is a popular model to model the interaction of visible light with objects in the environment and representing the image that is captured by a camera. Light field is a very important conceptual tool in understanding visible light image formation and also in rendering in computer graphics. Traditional light field represents the real-valued intensity of the light per unit solid angle as a function of three-dimensional viewing position and two-dimensional viewing angle, $R(u,v,w,\alpha,\beta)$, where $(u,v,w)$ is the position and $(\alpha,\beta)$ is the pair and azimuth and elevation angles respectively of the viewing direction. Additionally describing the light field as a function of wavelength and polarization has also been considered [??]. With evolution of modern applications which require to image the transient light transport, $I(x,y,t)$ led to describing light field as a function of time too in addition to above parameters.
%
%The complex-valued complex amplitude of RF light as a function of three-dimensional viewing position, two-dimensional viewing angle and time is surprisingly amenable to mathematical treatment similar to that of light field. We call this RF light field $R(u,v,w,\alpha,\beta,t)$, where $(u,v,w)$ is the position and $(\alpha,\beta)$ represent viewing direction as before and $t$ is time. Note that unlike light field which is real-valued, RF light field is complex valued.
%
%\subsection{Kajiya equation for RF light field}\label{sec:propagation}
%Light field is described using a simplified version of the rendering equation [??] popularly known as Kajiya equation. The equation dsicretizes the object space into small patches. The light field at each patch is described as a combination of direct emissive light field from the light source and global component from the light propagation from other light patches. For example, consider the light field at the patch indexed by $j$ in Fig??. $E[j]$ is the direct component from the light source. $\rho(j,k)$ represents the amount of irradiance from patch $k$ contributes to light field at path $j$ as a fraction of the light field at patch $k$. $\rho(j,k)$ includes the bidirectional reflectance distribution function which is a function of viewing angle from patch $k$ and considers the visibility between the two patches. So, the light field at patch $j$ can be written as superposition of the direct light field it receives from emissive sources $E[j]$ and $\rho(j,k)$ fraction of light from each of the other patches $L[k]$,
%\begin{equation}\label{eq:kajiya}
%L[j] =  E[j] + \sum_{k} \rho(j,k) L[k].
%\end{equation}
%
%The rendering equation has been the staple way to render the light field and for conceptually describing the light field in a scene. The equation has also been adapted to describe the light field as a function of time, $L[j,t] =  E[j,t] + \sum_{k} \rho(j,k) L[k, t - d_{jk}]$, where $d_{jk}$ is the time of propagation between the patches. This updated equation takes into account the finite speed of light and how the global component evolves with time providing access to image $I(x,y,t)$ that captures transient light transport. 
%
%Consider RF light field when the scene is illuminated by a RF light source as described in Sec.~\ref{sec:source}. So, the light source emits a time-dependent field. For this discussion, consider only one modulation frequency as each frequency of illumination can be treated differently.  We can consider same patches as described before in Fig?? and assume that the light source is a RF light source emitting $a_f \mathrm{e}^{(i 2 \pi (f_c + f) t + \phi)}$.  Consider steady state RF light field where the RF light source illuminated the scene long enough that the initial transients die off. Then the RF light field at any patch is sum of the direct emissive RF light field from the RF light source and a global component due to the RF light propagation from other patches.
%
%The direct component of RF light field at patch $j$, $E[j]$, is given by $a_f \mathrm{e}^{(i 2 \pi (f_c + f) (t - d_{pj}) + \phi  )} \frac{\rho(p,j)}{d_{pj} c}$, where $d_{pj}$ is the time of propagation between the two patches and $\rho(p,j)$ is a complex number indicating the fraction of complex-valued illumination that contributes to the RF light field at patch $j$. It includes the complex-valued bidirectional reflectance distribution function which is a function of viewing angle from patch $k$ and considers the visibility between the two patches. BRDF is complex because the both the amplitude and phase of the signal from a source or a patch are affected by the direction of emanation of RF light from the source or the patch. Notice how the light field at the patch $j$ is a complex sinusoidal signal with the same frequency. However, the complex attenuation multiplying the complex sinusoid changes by a factor of $\mathrm{e}^{(-i 2 \pi (f_c + f)d_{pj}  )} \frac{\rho(p,j)}{d_{pj} c}$. 
%
%Similarly, the light propagating from another patch $k$ to the patch $j$ changes the complex attenuation multiplying the complex sinusoid at the patch $k$ by a factor of $\mathrm{e}^{(-i 2 \pi (f_c + f)d_{kj} + i\phi  )} \frac{\rho(k,j)}{d_{kj} c}$. So, the RF light field which is nothing but sum of direct component and contributions from all the patches can be written as
%\begin{equation}\label{eq:kajiya_rf}
%L[j,t] =  E[j,t] + \sum_{k} \frac{\rho(k,j)}{d_{kj} c} L[k,t] \mathrm{e}^{(-i 2 \pi (f_c + f)d_{pj} )}.
%\end{equation}
%
%It is important to note the difference between steady state rendering equation for visible light, Eq.~\ref{eq:kajiya}, and the time dependent rendering equation for RF light, Eq.~\ref{eq:kajiya_rf}. In steady state Kajiya equation for light, the time of propagation information is completely lost. It is as if the light travels at infinite speed, i.e., the equation would have been the same irrespective of the distance between the patches. However, because RF light field is complex, the time of propagation information is retained in the rendering equation in the phase term. Therefore, even from the steady state rendering equation for RF light, it is possible to infer how the RF light may have propagated during the transients.  We will provide a more detailed initial exploration in the later sections.
%

%\subsection{Signal reception}\label{sec:demod}
%A simple photodetector integrates the light field across all dimensions to generate one signal value. The standard 2D cameras capture only a 2D projection of the light field by integrating along other dimensions. Ultrafast cameras that image the transport of light capture 3D projection of the light field including the time dimension. 
%
%Time-of-flight cameras capture a 2D projection of the light field. But in time-of-flight cameras, the light-field varies with time even in steady state because of the amplitude modulation at the light source. So, the ToF camera captures a time series of 2D projections of the light field. The phase of the captured sinusoidal amplitude modulated light contains the time-of-flight information of interest. However, the frequency of modulation is typically on the order of 10s of MHz where as images can only be captured by conventional solid state imagers at a rate of only 10s of Hz. Time-of-flight cameras perform a pretty neat trick to overcome the limitation. 
%
%Before being digitally sampled, the received signal is demodulated with the same amplitude modulation signal that the light source used. If the transmitted light has undergone a time of flight of $\tau$, then the received intensity is $g(t) = a \sin(2 \pi f (t - \tau) + \phi)$. The resultant signal after demodulation is
%\begin{equation}\label{eq:demod}
%\begin{aligned}
%& g(t) \sin(2 \pi \hat{f} t + \hat{\phi} ) = a \sin(2 \pi f (t - \tau) + \phi) \sin(2 \pi \hat{f} t + \hat{\phi} ) \\
%&= a \sin(2 \pi (f-\hat{f}) t  - 2\pi f \tau + \phi - \hat{\phi} ) \\
%& +  a \sin(2 \pi (f + \hat{f}) t  - 2\pi f \tau + \phi + \hat{\phi}).
%\end{aligned}
%\end{equation}
%The modulation and demoduation frequencies are $f$ and $\hat{f}$ respectively. The modulation and demodulation phases are $\phi$ and $\hat{\phi}$ respectively. In a typical Time of flight camera where the light source and the sensor are colocated and the modulation and demodulation signals are generated from the same clock source, the modulation and demodulation frequencies are one and the same. 
%
%Moreover, the samples of the signal are obtained by integrated the above demodulated signal over the exposure time. The exposure time acts as a low-pass filter and as long as the exposure time is significantly larger than the modulation/demodulation frequency, the high frequency term can be ignored and the integrating Eq.~\ref{eq:demod} over the exposure time results in 
%\begin{equation}
%a \sin (- 2\pi f \tau + \phi - \hat{\phi}),
%\end{equation}
%which clearly is a function of the ToF and relative phase of modulation and demodulation frequencies. By selecting four different values for the relative phase, which can be done because the modulation and demodulation signal sources share the clock source, one can resolve the value of ToF, $\tau$.
%
%In RF sensors, each antenna is analogous to a photodetector in that it generates a single value to represent the captured RF light field. Similar to photodetectors, the antennas have a field of view and their sensitivity is a function of the direction of the incoming RF light. The process of obtaining the signal, however, is close to the signal generation in ToF camera sensor rather than a simple integration as performed by a photodetector. Remember that the RF light source too produces a time varying RF light signal creating a time-varying RF light field. Similar to ToF cameras, the time of propagation values are embedded in the phase of the received signal. The frequency of illumination is in order of GHz but conventional RF transceivers can only sample at the rate of 10s of MHz. RF transceivers use the same trick as a ToF camera to overcome the limitation.
%
%Before being digitally sampled, the received signal is demodulated with the same amplitude modulation signal that the light source used. If the transmitted light has undergone a time of flight of $\tau$, then the received RF signal is $g(t) = a \mathrm{e}^{(2 \pi f (t - \tau) + \phi)}$. The resultant signal after demodulation is
%\begin{equation}
%\begin{aligned}\label{eq:demod_rf}
%& g(t) \mathrm{e}^{-(i2 \pi (\hat{f_c} + \hat{f}) t + i\hat{\phi})}  = a \mathrm{e}^{(i2 \pi (f_c + f) (t - \tau) + i\phi)} \mathrm{e}^{-(i2 \pi (\hat{f_c} + \hat{f}) t + i\hat{\phi})}   \\
%& = a \mathrm{e}^{-(i2 \pi (f-\hat{f} + f_c-\hat{f_c}) t  - i2\pi (f_c + f) \tau + i\phi - i\hat{\phi} )} \\
%& +  a \mathrm{e}^{(i2 \pi (f + \hat{f} + f_c + \hat{f_c}) t  - i2\pi (f_c + f) \tau + i\phi + i\hat{\phi})}.
%\end{aligned}
%\end{equation}
%
%
%In RF, the light source and sensor are typically different devices and it is not possible them to  share clock. The frequencies used for modulation/demodulation can be estimated and calibrated for using simple standard procedures~\cite{schmidl1997robust}. However, the relative phase between the signal used at the source modulation and the signal using at the sensor for demodulation is unknown and cannot be controlled as clocks constantly drift. So, $f$ and $\hat{f}$ can be assumed to be the same but not $\phi$ and $\hat{\phi}$.
%
%Similar to ToF camera, the samples of the signal are obtained by passing the above demodulated signal through a low-pass filter. So, the high frequency term can be ignored and the resulting signal is, 
%\begin{equation}
%a \mathrm{e}^{ i(- 2\pi (f_c + f) \tau + \phi - \hat{\phi}) },
%\end{equation}
%which clearly is a function of the ToF and relative phase of modulation and demodulation frequencies.
%
%The similarities and differences between RF light and visible light in signal generation, propagation, image formation, and sensing devices is highlighted in Table~\ref{compare}.
%
%\begin{table*}[ht]
%\begin{center}
%    \caption{Comparison of visible light and RF light sensors}
%\label{compare}
%
%\small{
%    \begin{tabular}{ | p{3.5cm} | p{6.0cm} |  p{6.8cm} |}
%    \hline
%     & \textbf{Visible light} & \textbf{RF light} \\ \hline
%     Wavelength & 100s of nms & few cms \\ \hline
%    Sensors & 	 Photodetectors  & Antennas \\ \hline
%    Number of sensors & Few millions & 3-4 in conventional devices \\ \hline
%    Coherent signal generation & Hard, only done for lasers & Easy, done using a simple oscillator \\ \hline
%    Modulation  & Amplitude only & Both amplitude and phase \\ \hline
%    Generated signal & $a_f \sin (2\pi f t + \phi)$, real-valued, for ToF cameras & $ a_f \mathrm{e}^{(i 2 \pi (f_c + f) t + i\phi)}$, complex-valued \\ \hline
%    Modulation frequency, $f$ & 10s of MHz & 10s of MHz \\ \hline
%    Sampling frequency & 10s of MHz & 10s of Hz \\ \hline
%    Carrier frequency  & few 100s of THz & few GHz \\ \hline
%    Carrier phase & None, due to incoherent illumination sources & Yes, and modulated \\ \hline
%    Free space propagation & $\frac{1}{r} a_f \sin(2 \pi f t + \phi - 2 \pi f \frac{r}{c})$  &  
%    $\frac{1}{r} a_f \mathrm{e}^{(2 \pi (f_c + f) t + \phi - 2 \pi (f_c + f) \frac{r}{c})}$ \\ \hline
%    Light field & $L(x,y,z, \theta, \rho, t, f)$, real-valued radiance  & $L(x,y,z, \theta, \rho, t, f)$, complex-valued RF light amplitude \\ \hline
%    %Kajiya equation, steady state & $L[j] =  E[j] + \sum_{k} \rho(j,k) L[k]$ & $L[j] =  E[j] + \sum_{k} \rho(j,k) L[k] \mathrm{e}^{(-i 2 \pi (f_c + f)d_{pj} )}$  \\ \hline  
%    Propagation time information in rendering equation & Lost & Embedded in phase \\ \hline  
% %   BRDF & Real-valued & complex-valued   \\ \hline  
% %   Kajiya equation, time-dependent  & $L[j,t] =  E[j,t] + \sum_{k} \rho(j,k) L[k, t - d_{jk}]  $ & $L[j,t] =  E[j,t] +  \sum_{k} \frac{ \rho(j,k)}{d_{jk} c}  L[k, t] { \mathrm{e}^{(-i 2 \pi (f_c + f) d_{jk} )} }  $  \\ \hline
%    Image formation at the sensor & Integration for photodetectors, Demodulation and low-pass filtering for Time of flight sensors & Demodulation and low-pass filtering \\ \hline
%    
%	Demodulated signal & $g(t) \sin (2\pi f t + \hat{\phi})$, g(t) is the received signal incident on the sensor in ToF camera &  $g(t) \mathrm{e}^{ (-i2\pi (f_c + f) t + \hat{\phi})}$, g(t) is the received signal incident on the sensor   \\ \hline  
%    
%    Phase used for signals used in modulation and demodulation & Can be finely controlled in conventional active imaging systems like ToF cameras where the light source and sensor are colocated & No control as the light source and sensor are separate devices in conventional RF systems \\ \hline
%    
%    Lens & 	 Yes & No \\ \hline
%    \end{tabular}
%}
%    
%\end{center}
%\end{table*}



 
%Discuss multipath, scattering - a phenomenon that affects both light and RF with similar mathematical equations. Again, the wavelength variable leads to fast decrement in energy due to scattering. 
%
%Discuss the differences in terms of occlusion, isotropy, specularity between RF and light.








%\section{Emerging RF cameras}
%As discussed in Sec.~\ref{sec:model}, the signal generation and image formation in visible light sensors and RF sensors can be described using strikingly similar mathematical machinery once we replace the photodetectors for antennas and the light field for complex RF amplitude. This lends us the tools to understand several computational imaging techniques in visible light and RF light that \textit{compute} new images from the sensor measurements. However, compard to visible light cameras, RF sensors have a distinct advantage of being able to generate phase-coherent RF light which can be modulated in both amplitude and phase domains, while RF sensors have a distinct disadvantage of having to work with limited number of sensors in the physical array and lack of lens. The lack of lens and small number of physical sensors severely limits RF sensors from achieving high resolution imaging/sensing.
%
%
%\subsection{Challenges}
%\textbf{Small physical sensor array: }In a visible light camera, the physical sensor array consists of millions of photodetectors. Image formed by a standard camera is nothing but a two dimensional representation of intensity of light incident along different directions at the camera. Each photodetector provides a single measurement. But the measurement from one pixel provides a different combination of intensities of the pixels of the physical world. The closer the directions of incident light that can be decoupled and represented as two different pixels in an image, the higher the resolution of the resultant image. A densely packed physical array of sensors enables capture the same physical scene with more number of pixels. This makes a large sensor array an important part of visible light cameras for high resolution. 
%
%However, RF sensors have very small number of antennas, which perform the analogous function of photodetectors in a camera. For example, ubiquitous WiFi devices have just 3-4 antennas. Similarly, the conventional autonomous radars have only 3-4 antennas. Even complicated, non-commercial, research systems used for communication and imaging purposes can afford atmost few tens of antennas. The complexity and cost of building Rf systems with a large number of antennas, each attached to its own transceiver circuits that measure the signal captured by the antenna, makes it almost infeasible to build RF cameras with large physical sensor arrays like a camera.
%
%
%\textbf{No lens: }In a visible light camera, lens perform an important function of decoupling the light that is incident on the lens from all the directions so that the light from one direction falls on one photodetector alone. A conventional sensor array, even if it consists millions of pixel sensors, it cannot achieve high resolution if the lens is of poor quality. This is because lens directs the light from one direction to multiple pixels resulting in blurred pixels with contributions from light coming from different directions.
%
%RF sensors do not have any lens. So, the signal at any of the antennas is sum of RF light coming from all the directions. So, there is no lens counterpart in RF sensors that map the pixels of the physical world to the pixel sensors so that the RF light from one pixel in the physical world contributes to only one antenna. The lack of such lens kind of acts in favor of RF imaging because, since there are very small number of antennas in RF sensors and a focusing device like a lens would only capture a small portion of the physical scene. Due to the lack of lens, the pixel sensors, which are the antennas, capture the information of all objects in the physical scene. However, the problem of recovering the image from the measurements generated by antennas, which contains a combination of RF light from all the objects in the physical scene, is challenging. 
%
%
%\textbf{Decoupled illumination source and camera: }Visible light cameras that capture information of intensity of light as a function of time in addition to as a function of the direction of incident light, have the illumination source and the camera sensor at the same location and share the clock. Generating signal from the same clock helps in making the phase used in modulation and demodulation of the signal the same. There are RF sensors like radars, where the illumination source and receiver are co-located and their oscillators are tightly coupled. However, in a more general setting, the illumination source and the receiver need not be co-located. For example, consider ubiquitous RF system like WiFi, where a WiFi signal source like one's cellphone is different from the WiFi signal receiver like a WiFi router. 
%
%Developing systems with decoupled source and receivers offers greater flexibility, enables novel applications and expands the kind of devices on which imaging can be enabled. However, with it comes the challenge of recovering ToF from systems where the light source and the receiver have clock offset making the estimated ToF values error-prone.
%
%%Assumptions like specularity, isotropy and sparsity of reflectors, and other limiting models of how the RF signals interact with the environment (Model Mismatch) 
%
%\subsection{Approaches}
%Significant advances in RF imaging systems that overcome above challenges have made it possible to achieve a subset of important applications of high resolution imaging. We hypothesize that these emerging advances, among others, enable generation of high resolution RF imaging. 
%\subsubsection{Extending sensing along other dimensions}
%By providing intensity of light coming from one direction, each pixel sensor in a traditional camera is essentially providing one specific linear combination of intensities of the pixels of the physical world. However, one does not need to have multiple pixels to provide multiple linear combinations. One can exploit sensors along other dimensions to provide multiple linear combinations, thus achieving high resolution imaging. 
%
%For example, single pixel imagers illuminate the scene with different patterns of light and the pixel measurement obtained for each pattern provides one linear combination of intensities of light~\cite{satat2017lensless}. So, when constrained by limited physical sensor array, multiple measurements are obtained along time dimension by exploiting the use of different patterns of light illumination. 
%
%Recent approaches in RF cameras explored exploiting sensors along non-physical dimensions to extract multiple measurements to enable high-resolution applications. For example, SpotFi~\cite{kotaru2015spotfi} explored using multiple frequencies of illumination to provide multiple combinations of the ToF values of RF light source and the reflectors in the environment. xdTrack ~\cite{xie2016xd} and WiCapture~\cite{kotaru2017position} used further extended it by using multiple measurements across time in addition to using multiple frequencies to exploit the different combinations provided by moving reflectors or a moving RF light source.
%
%The non-physical sensing dimension ideas go beyond finding ToF accurately for active light sources. For example,~\cite{ma2018enabling} and~\cite{radarBack} used large number of illumination frequencies, provided by high bandwidth systems like radar, to find the ToF of smart reflectors, like RFID tags, that do not actively generate light, 
%
%In RF imaging, SAR (Synthetic Aperture Radar) uses the fact that a moving RF light source changes the ToF of the signal from the RF light source to each of the pixels of the image~\cite{fu2018simultaneous}. So, limited physical array is overcome by collecting measurements on a virtual array obtained by moving the physical antenna array. In InSAR (Inverse Synthetic Aperture Radar) techniques, the moving reflector is used to create the virtual antenna array because as the reflector moves, the ToF from the RF light source to each of the pixels on the moving reflector changes creating multiple combinations of the intensity of the reflected RF light~\cite{chen2014inverse, adib2013see}.
%
%These include some dimensions but more dimensions are ripe for exploration. For example, projecting different patterns of RF light which are spatially different, using polarization, developing potential coded apertures all provide attractive options to generate a large number of sensor measurements.
%
%
%%
%%Exploit sensors along other dimensions. For example, multiple frequencies of illumination, passing the illumination through multiple projection masks, using the moving reflectors themselves to create multiple independent frequency measurements.
%%
%%\begin{equation}
%%\mathrm{e}^{i 2 \pi f (\tau + \phi) }
%%\end{equation}
%%
%%Make a diagrammatic representation with reresenting complex exponentials as phasors.
%%
%%More number of sensors results in more phasors and help in making the sum of phasers go to 0.
%%
%%More number of far away phasors helps in making sum of phasors go to 0 faster.
%%
%%This can be seen in other aproaches, for example, in radar sensing the resolution is $2/N$ where $N$ is number of sensing elements.
%%
%%You can change ToF $\tau$ by using multiple transmitter and receiver elements.
%%
%%If you tease apart signal from a moving reflector, it will create multiple time of flight measurements too.
%%
%%If you can tease apart signal from multiple reflectors, each reflector provides an estimate of clock offset. 
%%
%%Examples of these approaches include SpotFi, WiCapturem medical implant paperm Fadels rfid paper, Ayush Bhandaris paper with multiple frequencies to overcome multipath, prof. Raksar's paper to use reflections for clock offset.
%%
%%
%
%
%
%
%
%\subsubsection{Deep learning as computational lens}
%In the absence of physical lens that maps the pixels of the physical world at different directions to different pixels of an image, computational algorithms provide a way to decouple the signal coming from different directions. In visible light domain, lensless single pixel imagers resort to compressive sensing techniques to recover the signal incident along different directions by using a linearly independent set of combinations of the intensity of the reflections from different pixels of the physical world. 
%
%Even when lens are present, computational algorithms like super-resolution algorithms have also found use in ToF cameras to overcome inaccurate ToF measurements in complex scenes, e.g., when translucent surfaces are present. Remember from Sec.~\ref{sec:sensor} that the demodulation process in a ToF sensor assumes that there is a single reflector in any direction and the measurement provided by the corresponding photodetector is nothing but the sinusoid of ToF value to that reflector scaled by a known constant. However, when multiple reflectors are present in the same direction due to the presence of translucent surfaces, then the demodulation process results in sum of sinusoid signals, each with a different accumulated phase due to different distances traveled. The ToF value obtained by assuming that there is a single reflector will be error-prone. To overcome the inaccurate measurements due to multiple reflectors in the same direction, the ToF camera emits multiple frequencies of illumination and the processes the measurements obtained through super-resolution algorithms like MUSIC~\cite{schmidt1986multiple} to recover the image, $I(x,y,t)$ of interest~\cite{bhandari2014resolving, bhandari2014resolving2}.
%
%Similarly, in RF camera applications, compressive sensing~\cite{donoho2006compressed, candes2014towards} and other super-resolution algorithms like MUSIC have been explored to provide computational lens to RF cameras and is still an active research area. For example, WiDeo~\cite{joshi2015wideo}, a RF-based ToF imaging system with co-located RF light source and sensor, uses compressive sensing to decouple the signal coming from different reflectors. Note that unlike traditional ToF cameras, where a lens makes sure that the reflectors that contribute to the light detected by a photodetector are all coming from same direction, the signal detected by RF antennas is contributed by light incident from all the directions from all the reflectors. By decoupling the ToF of light coming from different reflectors, WiDeo measures the ToF of all the reflectors. To make the problem tractable,~\cite{joshi2015wideo} removes any signal coming from  stationary reflectors by doing background subtraction, and then, the compressive sensing only needs to decouple the signal from the moving reflectors.
%
%Similarly, ArrayTrack~\cite{arraytrack} and SpotFi~\cite{kotaru2015spotfi} used super-resolution algorithms like MUSIC~\cite{schmidt1986multiple} to decouple the signal from coming different reflectors and from the RF light source itself. The goal of these systems is, however, to only identify the signal from the RF light source itself, that has not undergone any reflections as the purpose of these systems is to locate the position of the RF light source. Once the signal along all the directions has been obtained, then the position information of the RF light source is obtained by analyzing the signal coming from the direction with the smallest ToF, as the signal that did not undergo any reflections has the smallest ToF in typical scenarios.
%
%However, all these approaches can be classified as model-based approaches. Compressive sensing and other super-resolution algorithms like MUSIC assume a model through which the environment affects the signal as they traverse though the environment from the RF light source to the RF sensor. Specifically, they assume that RG light follows ray propagation model, and that there are a small number of specular reflectors in the environment (typically 2-8 reflectors~\cite{kotaru2017position, kotaru2015spotfi}) and that there are no other objects in the environment. The reflectors are further treated as isotropic with same reflectivity in all the directions and at all the points on the reflector, i.e., the reflectors have same scattering function irrespective of viewing angle.  
%
%The modeling-based approaches then try to invert the non-linear, non-convex model to recover the ToF of different reflectors and the ToF of the RF light source by using obtained RF image and the underlying simplified model. Modeling based approaches are brittle and falter in the presence of mismatch between the model used for inversion and the actual model through which the measurements are formed [??]. However, the real environments are very complex with scattering, diffraction and irregular surfaces as described by the conceptual equations in Sec.~\ref{sec:propagation}. However, models accounting for these phenomenon are very complex and attempts to solve them can be computationally intractable. So, using approximate models is results in a significant model mismatch.
%
%More recent computational imaging approaches use deep learning to overcome the `model mismatch' problem. The algorithms that estimate the desired output of the high resolution imaging application are developed from observing lots of data rather than by inverting a simplistic model about how the signal interacts with the environment. One can potentially observe data and make modifications to the model to provide greater accuracy in high resolution imaging application of interest. However, emerging deep learning research and practice provides simple frameworks~\cite{abadi2016tensorflow, paszke2017automatic} to achieve the same from the given data making it an attractive approach to data-based/ data-educated algorithms.
%
%In visible light cameras,~\cite{satat2017object} uses deep learning approaches to overcome model mismatch created through uncalibrated sensors and scattering. In RF imagers, emerging approaches are exploring deep learning for several high resolution imaging applications like finding the location of a RF light source~\cite{singleWifi} and to recover the human pose using RF images ~\cite{zhao2018through} and to track the moving reflectors like breathing abdomen~\cite{yue2018extracting}. Deep learning based approaches significantly improved the localization and imaging resolution by doing away with simplistic models.~\cite{singleWifi} showed that combining deep learning based computational lens coupled with exploiting sensors in non-physical dimensions enables applications like localizing the RF light source with centimeter-scale accuracy.
%
%
%
%%Use deep learning approaches to overcome the `model mismatch'.
%%
%%Model based appraoches make simple approximations that the waves follow ray, propagation model, the reflectors are isotropic and specular, reflectors have same scattering function irrespective of viewing angle.
%%
%%Model based approaches like compressive sensing falter in the presence of mismatch. Consider where propagation model is a more realistic \textit{Wiener model}. Localization results start to deviate from ideal.
%%
%%The real environments are even more complex with scatttering and irregular surfaces.
%%
%%Examples include WiFi deep learning paper, Dinas CVPR paper, simulation based deep learning ToF paper. 
%
%
%\section{Applications}
%By enabling above approaches to enable high resolution sensing on the images captured by RF cameras, one can enable several important applications. The model of imaging developed in Sec.~\ref{sec:model} is sufficiently general and powerful enough to describe image formation in RF systems in multiple spectrums including RFID, WiFi, cellular, ultrawideband and millimeter-wave radars. We will now discuss three broad applications for high resolution imaging.
%
%\noindent{\textbf{Localizing active RF light sources: }}
%GPS has revolutionzed the way we travel by providing a powerful tool for navigation. However, a GPS receiver on phone has an error in localizing itself on the order of 3-10 meters and GPS system and algorithms used for localization fail in presence of occlusion like walls or in the presence of a large number of reflectors in the environment. Ability to localize a RF light source or a RF sensor with extremely high resolution of few millimeters has huge implications and revolutionize several important applications.
%
%It is of extreme importance to locate and track active RF light sources with applications in human and robot navigation even through occlusions, tracking robots like Roomba across rooms in a house, tracking drones in challenging environments, and for enabling positioning for augmented reality and virtual reality accessories. These applications can be enabled by placing simple, cheap, commoditized RF light sources on these devices and using the images obtained on RF sensors to decouple the signal coming from different directions and recover the ToF from the light source with very high resolution.
%
%Further, LIDAR light sources and RF light sources like radar used in autonomous vehicles have so far constrained the light source and receiver to be at the same location sharing a common clock.  Consider the scenario where multiple autonomous vehicles are simultaneously operating on a road. Each vehicle has its own LIDAR and RADARs and the signals interfere with each other creating extremely noisy ToF measurements with catastrophic consequences. Having a single light source on the road and if only receivers in the cars operate, then multiple autonomous vehicles can simultaneously generate maps and navigate. However, clock asynchrony between the light source and receiver makes the ToF measurements meaningless. However, if we localize the active light source with a very high accuracy, then the direct path ToF between the RF light source and the sensor provides us with the necessary calibration required to correct the clock offset between the transmitter and receiver. In general, we believe that the ability to free the light source from the receiver creates new opportunities for new applications.
%
%Providing high-accuracy GPS like positioning capabilities that work through indoor occlusions has been a driving force in research for couple of decades. However, recent attempts at overcoming small number of antennas and limiting models that are based on sparse specular reflectors have shown great promise to achieve the same[??]. 
%
%
%
%\noindent{\textbf{Localizing passive RF markers: }}
%Several applications like tracking medical implants inside body and inventory tracking, we cannot afford to attach active RF light sources. Passive reflectors that modulate incident light in a smart way so that they consume very little power while still being able to differentiate their  reflected signal from the signals from other reflectors in the environment. High fidelity, low-cost continuous motion capture through occlusions for applications like remote holographic rendering still alludes us. Smart RF reflector based systems provides an attractive option for enabling the same. 
%
%For roads, all the signs and markings are made with retro-reflective paintings that are interpretable by humans alone. With the emergence of autonomous vehicles, using reflective markers in non-visible spectrums provides distinct advantages as these signs can be robustly interpreted by millimeter-wave radars, that are already available on these cars, even through fog and occlusions.
%
%Smart reflector systems like RFID systems have been plagued with small number of illumination frequencies and a small number of antennas. Recent approaches that illuminate the scene with large number of frequencies showed promise in achieving accurate ToF to the reflective markers. We believe that combining these approaches with deep learning based model-free methods will account for deficiencies in traditional modeling that are too simplistic to account for complex propagation of waves inside complex media like human body.
%
%
%\noindent{\textbf{Imaging passive reflectors: }}
%Imaging passive reflectors is the traditional application of imaging. Providing the intensity of the reflected RF light and the corresponding ToF of the reflectors is very useful in several applications as the absorption properties of the RF light differ significantly from visible light enabling imaging of reflectors that are occluded. For example, consider an autonomous vehicle moving through fog or imaging for concealed weapons in airports, imaging a human body for diagnostic purposes, a drone imaging the skies for traffic control with other drones. 
%
%Radars have long been explored for RF imaging but they have mostly created images with extremely poor resolution on order of several tens of centimeters [??]. Exploiting the imaging target's motion to create multiple combinations of intensity of the the reflected light of different patches of the target reflector provides a large number of measurements provides opportunity for high resolution imaging. This process, called as Inverse Synthetic Aperture Radar (InSAR) imaging, has long been in use in imaging objects on a conveyer belt where one knows the exact trajectory of different patches of the target reflector [??]. In a more natural setting, using a ToF camera like Kinect to obtain the trajectories of different patches of the target reflector that is moving frees the system from having to rigidly attach the target to a conveyer belt whose motion is perfectly known. 
%
%There are multiple scenarios that require imaging through an occlusion but having a camera is a strict no-no; for example monitoring gait or detecting elderly fall throughout home including bedrooms and bathrooms. Visual odometry based techniques, used in systems like Hololens, that navigate a camera by continuously taking pictures also poses a significant privacy threat. In those scenarios, instead of equipping the environment with a ToF camera like Kinect to obtain the ToF of moving reflector creating multiple measurements across time, multiple RF reflectors can be embedded into walls in the rooms that provide multiple combinations of the intensity and ToF of any target reflector. Multiple smart reflectors in the environment essentially create different patterns of reflected light creating different combinations of pixels of the physical world.
%
%
%RF systems imaging a passive reflector have long been crippled by  limiting assumptions like reflectors are isotropic, i.e., the reflectivity of a reflector is the same irrespective of the viewing angle and that the reflectivity of different patched on a target reflector is the same. Different antennas, whether physical or virtual antennas caused due to motion of target or the imaging sensor itself whose motion is known, have different viewing angles of a patch on the  target reflector. Applying deep learning to transfer the series of viewing angles of different antennas and the respective measurements obtained at the antennas to recover the intensity of reflected light in RF spectrum in different patches of the target reflector provides a promising alternative that overcomes the limitations of existing algorithms that rely on simplistic assumptions.
%
%
%
%
%
%%\section{Applications}
%%\textbf{Separating the light source and receiver in a ToF sensing system: }Computational imaging and radar imaging communities have so far constrained the light source and receiver to be at the same location sharing a common clock. Ability to free the light source from the receiver creates new opportunities for new applications. For example, consider multiple autonomous vehicles simultaneously operating on a road. Each vehicle has its own LIDAR and RADARs and the signals interfere with each other creating extremely noisy ToF measurements with catastrophic consequences. Having a single light source on the road and if only receivers in the cars operate, then multiple autonomous vehicles can simultaneously generate maps and navigate. However, clock asynchrony between the light source and receiver makes the ToF measurements meaningless. Use reflectors in the environment which all carry the same clock offset but different ToF to successfully remove the clock offset.
%%
%%\textbf{WiFi localization: }Very useful for tracking roombas across rooms, occlusion free virtual reality, tracking robots in industrial setting, and navigation. Explore using sensing dimensions by projecting different patterns of light like a single-pixel camera. Remove model mismatch by using deep learning. Can we do something about different antenna array geometries? Also applicable to ultrawideband and other RF frequency signal sources.
%%
%%\textbf{Imaging active light sources: }In localization systems like Oculus, only intensity of the light source is used for transferring the image to obtain the location and orientation of headset. Ability to extract phase information enables even more accurate localization with micrometers of accuracy. With such high accuracy, you can even transfer data using laser beams and photo-detectors with small active area of few tens of micrometers for high bandwidth data transfer like the virtual reality content over wireless optical link.
%%
%%\textbf{Motion capture: }High fidelity, low-cost Continuous motion capture through occlusions for applications like remote holographic rendering still alludes us. Visible light systems require retro-reflective markers to be worn. RF also has passive markers in the form of RFIDs. They have been plagued with small number of sensors. Increase number of sensors along frequency dimension.
%%
%%\textbf{Implants: } Implants are also energy-sensitive making active light sources as implants undesirable. Similar as above. Body scatters the RF signals. Borrow techniques computational imaging community to account for scattering effects. Use deep learning to account for model deficiencies.
%%
%%\textbf{Driving signs: }In addition to retro-reflective paintings that are interpretable by humans alone, can we use reflective RF markers that are interpretable by radars in mm-wave frequency range that are already available even through fog and occlusions? 
%%
%%\textbf{Single-pixel cameras: }Use multiple frequencies of illumination like they use in ToF cameras but apply it to single-pixel ToF cameras. Use deep learning to obtain ToF image. Doe invisible light also has model mismatch?
%%
%%\textbf{Imaging moving target: }Consider imaging concealed weapons. or imaging a human body for diagnostic purposes. The moving target creates multiple independent measurements with different values for ToF. You get different viewing angles resulting in signal according to scattering function. Use a camera to know viewing angles. Apply deep learning to transfer the series of viewing angles and the respective scattering function values obtained to recover the shape of the object.
%%
%%\textbf{Imaging from a moving sensor: }Consider a drone imaging the skies for traffic control with other drones. Or consider an autonomous vehicle moving through fog. The moving sensor creates multiple independent measurements with different values for ToF. With same argument as above, apply deep learning to recover the image.
%%
%%\textbf{Sub-surface imaging: }In inspecting buildings and imaging insides of human, account for scattering by borrowing computational imaging techniques.
%%
%%\textbf{Scenarios where you do not want a visible-light camera: }There are scenarios where you do not want to have a camera. Like gait monitoring in bathroom or support system for blind with a system that is not capturing constantly everyone. Create multiple measurements with multiple reflectors in the room. The reflectors can be smart even changing their beam directions. This is applicable even for odometry for applications like Hololens where you don't need to take pictures for visual odometry but still get high resolution RF images that are not interpretable by human.
%
%\section{Discussion}
%Sensing the signal coming from a source is more or less like a dual of focusing the signal at a particular location. Consider "Degrees of freedom" in focusing versus "degrees of diversity" in sensing. Focusing is used in communications to deliver signal to only some spatial locations thereby effectively using the available energy. It is also used in selectively heating the tissue in RF ablation. You can achieve it using only small number of sensors and using deep learning.
%
%Super-resolution and compressive sensing are ineffective due to model mismatch. Deep learning super-resoles inspite of model mismatch.
%
%Transfer learning has been phenomenal and eliminated the necessity for large datasets for every imaging problem as a model trained on large datasets has captured high-level features that are common to images. Even in RF, use transfer learning from datasets that are easy to create. 
%
%Beyond RF into how these principles apply in IR imaging, CT scan, THz imaging. 
%
%
%










==> arxiv_rfImaging /iterative.tex <==

\subsection{Iterative reflection}
In Fig.~\ref{fig:superpos}, we have illustrated simple scenes where different RF-light patches are not geometrically visible to each other. If different patches are visible to each other, then the signal undergoes multiple reflections. For completeness, we extend the above model to account for these multiple reflections. For example, in Fig.~\ref{fig:kajiya}, the RF-light emitted from the source $p$ reaches the patches $k$ and $j$. Let $L[j,t]$ is the multi-dimensional RF-light field incident at patch $j$ at time $t$. As established by Eq.~\ref{eq:patch_transform}, each patch $j$ simply transforms the incident RF-light field by $\alpha_j S_j cos(\theta_{kj})$ and the RF-light field is then transformed by free space propagation before it reaches patch $k$. Here, $S_j$ is the size of patch $j$, $\theta_{kj}$ is the propagation angle from patch $j$ to patch $k$ with respect to the normal of patch $j$, and $\alpha_j$ depends on the properties of material constituting patch $j$ and the wavelength. So, the RF-light field contributed from patch $j$ to patch $k$ can be written as $\frac{1}{d_{kj}}\rho[k,j] L[j, t- \frac{d_{kj}}{c}]$, where 
\begin{equation}\label{eq:rf_brdf}
\rho[k,j] = \alpha_j S_j cos(\theta_{kj}). 
\end{equation}

The RF-light field at patch $k$ due to all the light patches can then be summarized into the following equation:
\begin{equation}\label{eq:kajiya}
L[k,t] = E[k,t] + \sum_j g[k,j]\rho[k,j] L\big[j, t-\frac{d_{kj}}{c} \big]. 
\end{equation}
In Eq.~\ref{eq:kajiya}, $E[k,t]$ accounts for the direct component obtained at patch $k$ from the light source $p$ without interacting with any other objects. $g[k,j]$ is a geometric factor that equals $\frac{1}{d_{kj}}$ is patch $k$ is visible from patch $j$ and $0$ otherwise. Notice how Eq.~\ref{eq:kajiya} is an iterative equation with RF-light of a patch appearing on both sides of the equation. This equation is strikingly similar to rendering equation used in computer graphics literature and we delve more into this similarity in Sec.~\ref{sec:brdf}. 


\begin{figure}
  \centering
    \includegraphics[width=0.7\linewidth]{./figures/kajiya.pdf}
      \caption{Iterative RF-light transport when different RF-light patches are gemetrically visible to each other.}
      \label{fig:kajiya}
\end{figure}






\subsection{Relation to light field transformation in visible light}\label{sec:brdf}
In computer graphics literature limited to ray nature of light, the objects in the scene are divided into small light patches. The light field gets transformed due to properties of the reflector material and irregularities in the surface that lead to reflection in different directions. This transformation of the light field is captured by a quantity called as bidirectional reflectance distribution function (BRDF), which is the irradiance emitted from the patch as a function of the directions of incoming and outgoing light fields. For visible light, BRDF is a complex function because the wavelength is fraction of a micrometer. So, irregularities in a centimeter-sized light patches are much bigger than the wavelength and result in reflections in different directions depending on the irregularity profile. In contrast, BRDF for RF-light patches that can be approximated to wavelet sources is given by Eq.~\ref{eq:rf_brdf}.

Ability to apply simple wavelet approximation also offers advantage in terms of being able to represent wave phenomenon like diffraction. In traditional optics, Wigner Distribution Functions (WDFs) are calculated for every surface profile to calculate the transformation that the light field undergoes as it passes through a particular diffraction medium ??, which is inconvenient. In contrast, superposition of transformed RF-light field propagated from different wavelet sources automatically accounts for reflection, refraction, diffraction and interference phenomenon.

Iterative equation, Eq.~\ref{eq:kajiya}, written to account for multiple reflections is of the same form as classic rendering equation in computer graphics literature??. The rendering equation in Eq.~\ref{eq:kajiya} is time-dependant. RF-light field $L[k,t]$ is complex amplitude rather than intensity of light used in classic equation. BRDF $\rho[k,j]$ is a simple function for reasonably-sized patches. The geometric factor $g[k,j]$ is inversely proportional to the distance between patches rather than square of the distance used in classic equation.


==> arxiv_rfImaging /propagation.tex <==
\section{Propagation}\label{sec:free}

Amplitude of RF signal emitted from a point source falls off as $1/r$ as it travels a distance $r$ in free space. Further, the signal undergoes a delay of $r/c$, where $c$ is the speed of light, transforming the signal to $\frac{A}{r} \mathrm{e}^{ i2 \pi f (t - \frac{r}{c})}$. The signal propagates through spherical wavefronts. So, the RF light-field observed at a point $r \mathrm{\textbf{v}}$ with a point source located at the origin, with a unit vector $\mathrm{\textbf{v}}$ , is given by 
\begin{equation}\label{eq:free}
L[x, y, z, \xi, \psi, t , f ] = \frac{A}{r} \mathrm{e}^{ i2 \pi f t} \mathrm{e}^{- i2 \pi \frac{r}{\lambda}} g(\xi, \psi,  \mathrm{\textbf{v}}).
\end{equation}
In Eq.~\ref{eq:free}, $ (x,y,z) = r \mathrm{\textbf{v}}$ and $g(\xi, \psi,  r \mathrm{\textbf{v}})$ is a geometric factor that is 1 only if the direction determined by the angles of interest at the point, $(\xi, \psi)$ is along the unit vector $\mathrm{\textbf{v}}$ joining the source to that point. 

In visible light systems like those discussed in Sec.~\ref{sec:emitLight}, the intensity of the emitted light drops as inverse square of distance of propagation resulting in $\frac{A}{r^2} x(t - \frac{r}{c})$.






==> arxiv_rfImaging /receiver.tex <==
\section{Receiver}\label{sec:receiver}
As discussed in Sec.~\ref{sec:sensor}, each antenna sensor of a RF camera integrates RF light-field over all angles at the RF camera. However, an RF camera does not simply sample the resultant signal at different time instants. An RF camera multiplies the signal captured by antennas with a reference sinusoidal signal before integrating the signal over exposure time. This process is called demodulation. 

Let $L[x_k, y_k, z_k, \xi, \psi, t, f]$ be the RF light-field incident at an antenna located at $(x_k, y_k, z_k)$. The antenna of RF camera integrates RF light-field along all angles and then performs demodulation to obtain the image
\begin{equation}\label{eq:receiver}
I(x_k, y_k, z_k,f) = \int_T \Bigg( \int_{\theta,\psi} L[x_k, y_k, z_k, \xi, \psi, t, f]  \Bigg) \mathrm{e}^{-i2\pi f t - \phi},
\end{equation}
where $T$ is the integration time, and $\xi$ and $\psi$ are propagation angles at RF camera. The exposure time varies from a fraction of a microsecond in pulse-based radars to few microseconds in WiFi-based RF cameras. 

% Note that the time-dependent term in the RF signal is only $\mathrm{e}^{i2\pi f t}$, even as it propagates through free space and interacts with the environment as seen from Eq.~\ref{eq:free} and Eq.~\ref{eq:patch_transform}. So, Eq.~\ref{eq:receiver} can be simplified to 
% \begin{equation}\label{eq:receiver}
% I(f) = \int_T \Bigg( \int_{\theta,\psi} L[x_k, y_k, z_k, \xi, \psi, t, f]  \Bigg) \mathrm{e}^{-i2\pi f t - \phi}.
% \end{equation}

Notice that the sinusoidal signal used for demodulation $\mathrm{e}^{-i2\pi f t - \phi}$ has the same frequency as the signal used at the emitter. However, the phase of the sinusoidal signal can differ from that of the phase used in transmitted signal. In RADAR systems, both the emitter and receiver are on the same device  and share the same oscillator that generates the sinusoidal signal; so, in radars $\phi$ is 0. But in systems like WiFi, the emitter and receiver are separate devices and the relative phase $\phi$ between the sinusoidal signal used at the emitter and receiver cannot be controlled or known.

\subsection{Relation to receiver in visible light cameras}
In traditional cameras the light field is integrated during the exposure time. ToF cameras like Kinect perform a simple demodulation operation by multiplying the received signal with ${\sin(2\pi ft + \phi)}$ and then passing the resultant signal through a low pass filter by integrating the signal over exposure time $T$. $T$ is typically few milliseconds. The relative phase $\phi$ is known and accurately controlled as both the emitter and receiver are on the same device and share the oscillator generating the sinusoidal signal.


==> arxiv_rfImaging /relatedWork.tex <==
\section{Related Works}\label{sec:relatedworks}



\subsection{Cameras Beyond Visible Light}
Majority of imaging modalities are in the visible part of the EM spectrum. Additional imaging modalities that are not EM based include e.g. ultrasound and magnetic resonance imaging (MRI). Imaging with EM energy near the visible spectrum such as ultra violet (UV) and near infra red (NIR) is commonly achieved with Silicon detectors and traditional lenses. Imaging with shorter wavelengths includes X-Ray (with added modalities such as CT). Imaging with longer wavelengths include infrared, microwave~\cite{charvat2015time}, Thz~\cite{redo2016terahertz}, mm-wave~\cite{appleby2007millimeter, wei2015mtrack}, and RF~\cite{wallace2010analysis}. Overcoming the lack of high quality lenses and availability of dense detector arrays is usually achieved by raster scanning, bare sensor imaging~\cite{napier1983very}, and with compressive sensing~\cite{satat2017lensless}. In this work, our goal is to focus on imaging with longer wavelengths and RF in particular.


\subsection{Imaging with RF}

Imaging in RF spectrum has been widely explored for specialized applications. RADAR is the most known application of RF for sensing applications. Recently new applications emerged.

\textbf{Imaging Through Walls} leverages the fact that RF is not highly absorbed by common construction materials such as wood and drywall. Various works explored different parts of the RF spectrum such as ultrawideband~\cite{yang2005see, ralston2010real, peabody2012through} and WiFi~\cite{adib2013see}. Different applications include capturing the shape of a human~\cite{adib2015capturing, zhao2018through} and human computer interaction applications~\cite{bedri2015rflow}. 

%Recovery using multiple platforms~\cite{depatla2015x}


\textbf{Motion Tracking} is a specific instance of RF imaging. Because of the relatively longer wavelength it is usually hard to form images, and specific applications such as motion tracking~\cite{kotaru2015spotfi} are tackled directly. Tracking can be used for monitoring vital signs~\cite{adib2015smart}, or for human computer interaction~\cite{kotaru2017position,pu2013whole,joshi2015wideo}.

\textbf{Synthetic Aperture Radar (SAR)} overcomes the main limitation in forming an image with RF. Because of the long wavelength and size of detectors, a very large aperture is required which in practice is not feasible. SAR overcomes that challenge by forming a synthetic large aperture~\cite{ralston2010interferometric, chen2014inverse, holloway2017savi}.

The systems above provide application-specific description of RF imaging.  Here, we suggest a different perspective for imaging with RF. We expand fundamental concepts in visible light imaging systems like light-field to describe RF imaging systems. Our formulation accounts for wave effects like diffraction and interference which play a dominant role in RF imaging systems due to large wavelengths. Wigner Distribution Functions have been considered to describe wave effects in the context of light field for visible light~\cite{zhang2009wigner}. By expanding fundamental concepts in computational photography with visible light to RF, we expect that many novel RF imaging applications will emerge.


==> arxiv_rfImaging /resolution.tex <==

\begin{figure*}
\begin{subfigure}{.24\textwidth}
  \centering
    \includegraphics[width=1\linewidth]{./figures/apertureReq}
      \caption{Length of array required for achieving an angular resolution of 10 degrees as a function of frequency.}
      \label{fig:arrayRes}
\end{subfigure}
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
    \includegraphics[width=1\linewidth]{./figures/resolAchieved}
      \caption{Resolution of 10 cm long array as a function of frequency.}
      \label{fig:fixedArrayRes}
\end{subfigure}
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
    \includegraphics[width=1\linewidth]{./figures/minSurfRes}
      \caption{Resolution limit in imaging surface irregularities as a function of frequency.}
      \label{fig:surfRes}
\end{subfigure}
\hfill
\begin{subfigure}{.24\textwidth}
  \centering
    \includegraphics[width=1\linewidth]{./figures/tofRes}
      \caption{Time-of-Flight Resolution as a function of bandwidth.}
      \label{fig:tofRes}
\end{subfigure}
\caption{Analysis of resolution}
\end{figure*}

\section{Imaging Resolution}\label{sec:resolution}

In this section, we analyze the imaging resolution provided by a RF camera. The images produced at different antennas and at different frequencies is given by Eq.~\ref{eq:receiver}. The information of RF light-field as a function of propagation angles is embedded in that image information. But, it is not readily accessible, like in a traditional visible camera where a lens maps the signal from different scene points to different pixels in an image. So, computational algorithms like synthetic aperture radar are used to recover a more traditional representation of image, i.e., reflected intensity as a function of Cartesian coordinates of the imaged scene. We now analyze the resolution of such representation in simple two-dimensional scenes. However, the analysis can be extended to three-dimensional scenes.

\noindent\textbf{Aperture: } Consider a dense array of antennas in a linear array where adjacent antennas are separated by no more than half the wavelength of light. The length of the antenna array is called an aperture. As shown in~\cite{bouman2016computational}, the resolution with which signals from different angles can be resolved in a dense scene, i.e., the RF signal has significant value for every angle at the camera, is given by 
\begin{equation}\label{eq:array_res}
\mathrm{resolution} = \frac{\lambda}{\mathrm{aperture}}.
\end{equation}
The length of the array required for angular resolution of 10~degrees for different frequencies in RF spectrum in plotted in Fig.~\ref{fig:arrayRes}. Similarly, the resolution offered by a 10~cm array in different frequencies is presented in Fig.~\ref{fig:fixedArrayRes}. Note that in the algorithms used to achieve the resolution dictated by Eq.~\ref{eq:array_res}, it is assumed that the range to the object is very large when compared to the aperture. 

\noindent\textbf{Wavelength: }It is impossible to recover arbitrarily fine features like irregularities on a surface just by increasing the length of the antenna array. As shown in Fig.~\ref{fig:pointApprox}, if a patch of size one-tenth of wavelength or smaller is composed of uniform material, then the patch can be approximated by a wavelet point source. So, once the resolution dictated by Eq.~\ref{eq:array_res} reaches this limit, then increasing the array length does not enable to image finer surface irregularities. This is because there is no difference between such a surface and a point source. This limit in the resolution as a function of frequencies in radio spectrum is shown in Fig.~\ref{fig:surfRes}. We note that this limit is applicable only if the surface is composed of material with same RF properties. 

%For example, if there are two RF point sources separated by less than a wavelength, their positions can be uniquely recovered by observing the interference pattern in the image and by knowing that there are only two RF-light sources.


\noindent\textbf{Bandwidth: }The signal from different elements in a scene can also be resolved using Time-of-Flight. So, even if the signal from two elements in a scene have close-by angles with respect to the RF camera, they can be resolved in the time dimension. This is possible because the RF image is obtained at different frequencies. The time resolution as a function of bandwidth, i.e., the range of frequencies used in the imaging system, is shown in Fig.~\ref{fig:tofRes}. 


\noindent\textbf{Object size: }Small objects act as reflective diffractors and reflect in a diffuse manner. However, the amplitude of reflected light is small because the size of the object is small. Large reflectors reflect in a specular manner. Such that the intensity of light from the object is focused only in one direction and the signal is very small in all other directions. We analyze this interplay here by calculating amplitude of light reflected from an object. We consider a scenario where the emitter and the receiver are at the same location, like a RADAR. The object is placed parallel to the antenna array. The \textit{angle of the object} is defined as the angle of the vector joining the midpoint of the object and the midpoint of the array with respect to the normal of the antenna array. The frequency of the RF signal is set at 2.4~GHz. The object plane is assumed to be 4~m away from the RF camera plane.

\begin{figure}[h]
  \centering
    \includegraphics[width=0.8\linewidth]{./figures/objSize}
      \caption{Amplitude of the reflected signal as a function of the object size and angle of the object.}
      \label{fig:sameAngle}
\end{figure}

Fig.~\ref{fig:sameAngle} plots the amplitude of the RF signal obtained at the midpoint of antenna array. From the figure, we observe that when the \textit{angle of the object} is small, increasing the size of the object results in higher amplitude. However, if the \textit{angle of the object} is large, then the effects of increased size and increased reflector specularity tend to cancel out as the object size increases.


%10 cm is the size of typical phone, 40 cm is the size of a typical laptop or human and 4 m is the size of a typical wall. Note that the the examples like human and wall are provided just as intuitive cues for sizes; the plots in the Fig.~\ref{fig:sameAngle} are for objects made from same material of perfect conductor. 























==> arxiv_rfImaging /transformation.tex <==
\begin{figure}
  \centering
    \includegraphics[width=0.4\linewidth]{./figures/patch.pdf}
      \caption{RF signal from a patch is superposition of the signals from wavelet sources.}
      \label{fig:patch}
\end{figure}

\section{Transformation of RF light field}\label{sec:transform}
We will now represent the transformation of RF light-field when it reaches an object or obstruction. For example, consider the interaction of a spatially-uniform but time-dependent RF signal, $\mathrm{e}^{i2\pi f t}$, as it interacts with a thin patch of an object shown in Fig.~\ref{fig:patch}. The RF signal received at a point $P'$ is given by Rayleigh-Sommerfeld formula:
\begin{equation}\label{eq:rayleigh}
u(P') =  \int_S \mathrm{e}^{i2\pi f t} \alpha \frac{\mathrm{e}^{-i 2 \pi r / \lambda}}{r}  \cos(\theta)    ds,
\end{equation}
where $S$ is the surface of the patch, $r$ is the distance between an infinitesimal patch element $ds$ and $P'$, $\theta$ is the angle between the outward normal of the patch and the vector joining the patch element $ds$ to $P'$, and $\alpha$ is a weighting factor which depends on the properties of the material constituting the patch and the wavelength of light. The infinitesimal patch elements are called as wavelet sources. 




\begin{figure}
  \centering
    \includegraphics[width=0.8\linewidth]{./figures/huygens.pdf}
      \caption{Amplitude of signal from the patch versus the angle of propagation as a function of the patch width.}
      \label{fig:pointApprox}
\end{figure}


If the width of the patch is much smaller than the the distance between the patch and the receiver point $P'$, then the signal $u(P')$ from Eq.~\ref{eq:rayleigh} can be approximated by:
\begin{equation}\label{eq:simple_rayleigh}
u(P') = \mathrm{e}^{i2\pi f t} \alpha  {\mathrm{e}^{-i 2 \pi R / \lambda}} \frac{\cos(\theta)}{R} \int_S {\mathrm{e}^{i 2 \pi s \sin\theta / \lambda}} ds,
\end{equation}
where $R$ is the distance between the midpoint of the patch and the receiver point $P'$, $s$ is the distance from that midpoint to an infinitesimal patch element. The value of the integrand as a function of propagation angle $\theta$ for different sizes of the patch is provided in Fig.~\ref{fig:pointApprox}. The value is normalized by the integrand's value for $\theta=0$. One can clearly observe from Fig.~\ref{fig:pointApprox} that for a larger patch size (in relation to the wavelength), the signal obtained from a thin patch deviates more from that of an ideal wavelet source. If the width of the patch is less than one-tenth of the wavelength, one can approximate the patch by an ideal wavelet source. 

Evaluating Eq.~\ref{eq:simple_rayleigh} for such patches with size smaller than one-tenth of the wavelength results in 
\begin{equation}\label{eq:patch_transform}
u(P') = \mathrm{e}^{i2\pi f t} \alpha  {\mathrm{e}^{-i 2 \pi R / \lambda}} \frac{\cos(\theta)}{R} S,
\end{equation}
where $S$ is the size of the patch. By comparing Eq.~\ref{eq:patch_transform} and Eq.~\ref{eq:free}, one can interpret that each such patch multiplies the incident RF signal by propagation-angle-dependent term $\alpha S \cos(\theta)$, and then emits the resultant signal to be propagated in free space to reach $P'$.
%So, these patches can be treated as \textbf{RF-light field transformers} that transform the RF-light field by $\alpha S \cos(\theta)$ before emitting them for free space propagation.


\begin{figure*}
\begin{subfigure}{.31\textwidth}
  \centering
    \includegraphics[width=0.9\linewidth]{./figures/ref.pdf}
        \caption{Reflector}
        \label{fig:ref}
\end{subfigure}
\hfill
\begin{subfigure}{.31\textwidth}
  \centering
    \includegraphics[width=0.9\linewidth]{./figures/refDiff.pdf}
        \caption{Reflective Diffraction}
        \label{fig:refDiff}
\end{subfigure}
\hfill
\begin{subfigure}{.31\textwidth}
  \centering
    \includegraphics[width=0.9\linewidth]{./figures/diff.pdf}
        \caption{Transmissive Diffraction}
        \label{fig:Diff}
\end{subfigure}
\caption{RF images rendered using superposition of signals from discretized patches approximated as wavelet sources.}
    \label{fig:superpos}
\end{figure*}


Applying this interpretation automatically accounts for different wave effects like reflection, refraction and diffraction. For example, Fig.~\ref{fig:ref} shows the RF signal contributed at an array of points due to a large reflector of size 4~m present in the scene. The frequency of the signal used is 2.4~GHz corresponding to a wavelength of 12.5~cm. The object has been divided into patches of size 1~cm. One can observe that the wavefront arrives at different angles at different arrays of points which is intuitive because signal reflected from large objects follows Newtonian laws of reflection. If the object size is comparable to wavelength of light as in Fig.~\ref{fig:refDiff}, reflective diffraction is observed. Fig.~\ref{fig:Diff} considers a scene in which the source and the array of points are separated by a large object which has a small opening. The opening can be treated as a diffractor object and Eq.~\ref{eq:patch_transform} can be used for calculating signal passing through patches of this diffractor object. In this section, for simplicity, we considered only two-dimensional scenes. However, the concepts can be trivially extended to three-dimensional scenes.





RF signal incident from any angle at a patch reflects in all directions away from the interior of the patch according to Eq.~\ref{eq:patch_transform}. The ratio of reflected signal amplitude compared to incident signal amplitude is given by 
\begin{equation}\label{eq:rf_brdf}
 \alpha S \cos(\theta),
\end{equation}
which provides the reflectance function for RF. This is similar to the concept of BRDF in visible light. Note that this reflectance function for RF is a function of the outgoing direction alone and not the incoming direction. However, we note that this formulation for reflectance function is a result of simplistic model that does not account for sub-surface scattering. More complicated models that account for scattering and procedures for experimentally measuring them of real objects is beyond the scope of this paper and is part of future work.

Eq.~\ref{eq:patch_transform} shows the signal emitted from a patch for an incoming signal arriving from one direction. In general, RF light-field arriving at a patch has signal along multiple directions. The overall emitted RF light-field from the patch can be written as
\begin{equation}
L(x,y,z, \xi, \psi, t, f) = \rho(\xi, \psi) \int\displaylimits_{\xi', \psi'} L(x,y,z,\xi',\psi',t,f)  d\xi' d\psi',
\end{equation}
where $L(x,y,z,\xi',\psi',t,f)$ is the RF light-field incident along direction dictated by azimuth and elevation  angles $\xi'$ and $\psi'$respectively.  $\rho(\xi, \psi)$ is the reflectance function of the patch, Eq.~\ref{eq:rf_brdf}, evaluated along the direction dictated by angles $\xi$ and $\psi$. 













==> iterative.tex <==

\subsection{Iterative reflection}
In Fig.~\ref{fig:superpos}, we have illustrated simple scenes where different RF-light patches are not geometrically visible to each other. If different patches are visible to each other, then the signal undergoes multiple reflections. For completeness, we extend the above model to account for these multiple reflections. For example, in Fig.~\ref{fig:kajiya}, the RF-light emitted from the source $p$ reaches the patches $k$ and $j$. Let $L[j,t]$ is the multi-dimensional RF-light field incident at patch $j$ at time $t$. As established by Eq.~\ref{eq:patch_transform}, each patch $j$ simply transforms the incident RF-light field by $\alpha_j S_j cos(\theta_{kj})$ and the RF-light field is then transformed by free space propagation before it reaches patch $k$. Here, $S_j$ is the size of patch $j$, $\theta_{kj}$ is the propagation angle from patch $j$ to patch $k$ with respect to the normal of patch $j$, and $\alpha_j$ depends on the properties of material constituting patch $j$ and the wavelength. So, the RF-light field contributed from patch $j$ to patch $k$ can be written as $\frac{1}{d_{kj}}\rho[k,j] L[j, t- \frac{d_{kj}}{c}]$, where 
\begin{equation}\label{eq:rf_brdf}
\rho[k,j] = \alpha_j S_j cos(\theta_{kj}). 
\end{equation}

The RF-light field at patch $k$ due to all the light patches can then be summarized into the following equation:
\begin{equation}\label{eq:kajiya}
L[k,t] = E[k,t] + \sum_j g[k,j]\rho[k,j] L\big[j, t-\frac{d_{kj}}{c} \big]. 
\end{equation}
In Eq.~\ref{eq:kajiya}, $E[k,t]$ accounts for the direct component obtained at patch $k$ from the light source $p$ without interacting with any other objects. $g[k,j]$ is a geometric factor that equals $\frac{1}{d_{kj}}$ is patch $k$ is visible from patch $j$ and $0$ otherwise. Notice how Eq.~\ref{eq:kajiya} is an iterative equation with RF-light of a patch appearing on both sides of the equation. This equation is strikingly similar to rendering equation used in computer graphics literature and we delve more into this similarity in Sec.~\ref{sec:brdf}. 


\begin{figure}
  \centering
    \includegraphics[width=0.7\linewidth]{./figures/kajiya.pdf}
      \caption{Iterative RF-light transport when different RF-light patches are gemetrically visible to each other.}
      \label{fig:kajiya}
\end{figure}






\subsection{Relation to light field transformation in visible light}\label{sec:brdf}
In computer graphics literature limited to ray nature of light, the objects in the scene are divided into small light patches. The light field gets transformed due to properties of the reflector material and irregularities in the surface that lead to reflection in different directions. This transformation of the light field is captured by a quantity called as bidirectional reflectance distribution function (BRDF), which is the irradiance emitted from the patch as a function of the directions of incoming and outgoing light fields. For visible light, BRDF is a complex function because the wavelength is fraction of a micrometer. So, irregularities in a centimeter-sized light patches are much bigger than the wavelength and result in reflections in different directions depending on the irregularity profile. In contrast, BRDF for RF-light patches that can be approximated to wavelet sources is given by Eq.~\ref{eq:rf_brdf}.

Ability to apply simple wavelet approximation also offers advantage in terms of being able to represent wave phenomenon like diffraction. In traditional optics, Wigner Distribution Functions (WDFs) are calculated for every surface profile to calculate the transformation that the light field undergoes as it passes through a particular diffraction medium ??, which is inconvenient. In contrast, superposition of transformed RF-light field propagated from different wavelet sources automatically accounts for reflection, refraction, diffraction and interference phenomenon.

Iterative equation, Eq.~\ref{eq:kajiya}, written to account for multiple reflections is of the same form as classic rendering equation in computer graphics literature??. The rendering equation in Eq.~\ref{eq:kajiya} is time-dependant. RF-light field $L[k,t]$ is complex amplitude rather than intensity of light used in classic equation. BRDF $\rho[k,j]$ is a simple function for reasonably-sized patches. The geometric factor $g[k,j]$ is inversely proportional to the distance between patches rather than square of the distance used in classic equation.

